Economically Viable Randomness

We study the problem of providing blockchain applications with \emph{economically viable randomness} (EVR), namely, randomness that has significant economic consequences. Applications of EVR include blockchain-based lotteries and gambling. An EVR source guarantees (i) secrecy, assuring that the random bits are kept secret until some predefined condition indicates that they are safe to reveal (e.g., the lottery's ticket sale closes), and (ii) robustness, guaranteeing that the random bits are published once the condition holds. We formalize the EVR problem and solve it on top of an Ethereum-like blockchain abstraction, which supports smart contracts and a transferable native coin. Randomness is generated via a distributed open commit-reveal scheme by game-theoretic agents who strive to maximize their coin holdings. Note that in an economic setting, such agents might profit from breaking secrecy or robustness, and may engage in side agreements (via smart contracts) to this end. Our solution creates an incentive structure that counters such attacks. We prove that following the protocol gives rise to a stable state, called Coalition-Proof Nash Equilibrium, from which no coalition comprised of a subset of the players can agree to deviate. In this stable state, robustness and secrecy are satisfied. Finally, we implement our EVR source over Ethereum.

==> figures/framing_ethereum.tex <==
\begin{algorithm} %\caption{\label{proc} \textsc{ProcessNode }} 
% 	\caption*{\textbf{The escrow account $\G$}}
	\captionof{figure}{\label{fig:framing_ethereum}Practical Framing (in Ethereum)}
	\begin{algorithmic}[1]
    
    	\footnotesize
    
        % \Statex Init: 
        % \Statex\hskip1.6em $accounts \leftarrow $ empty list 
        % \Statex\hskip1.6em $n,\leftarrow 0$
        % \Statex\hskip1.6em $X,x \leftarrow \bot$
        % \Statex\hskip1.6em $tout_1, tout_2$
        % \Statex\hskip1.6em $verCommit,verReveal \leftarrow false$
        % \Statex\hskip1.6em $stage \leftarrow \text{`registration'}$ 
        % \Statex
        
        % \Statex Let $FRAMING\_DEPOSIT$ be a constant.
        \Statex \red{A simplified version -- supports only the first user who invokes frameCommit(). A full version would support multiple users who try to frame.}
        
        \Statex \centerline{\normalsize\textbf{User}}
        \Statex - $pk$: the user's EOA identifier.
        \Statex 
        % \Statex
        \Statex\underline{function $\ascii{frame}(secret)$}
        \Indent
            \State $commit \leftarrow H(pk||secret)$
            \State $\E.\ascii{frameCommit}(commit, \$FRAMING\_DEPOSIT)$
            \State wait $tout_3$ steps \Comment{counteracts chain reorganization}
            \State $\E.\ascii{frameReveal}(secret,pk)$
        \EndIndent
        
        % \Statex \phantom
        \begin{center}
            {\normalsize\textbf{Smart contract $\E$}}
        \end{center}
        % \centerline{\normalsize\textbf{Smart contract $\E$}}
        \Statex - Auxiliary globals: $framingCommit$, $frameStart$.
        \Statex - $H$ is SHA-3 hash function.
         
        \Statex
        \Statex  \underline{function $\ascii{frameCommit}(commit, \$d)$} 
        \Indent
            \State ($balance = balance + \$d$)
            \State \textbf{if} $stage == \text{'pending'}$
            \Indent
                \State \textbf{if} not $cnd$ \textbf{and} $d == FRAMING\_DEPOSIT$
                \Indent
                    \State $frameStart \leftarrow clock.now$
                    \State $framingCommit \leftarrow commit$
                    \State $stage \leftarrow \text{'pending framing'}$
                \EndIndent
            \EndIndent
        \EndIndent
        
        \Statex  \underline{function $\ascii{frameReveal}(secret,pk)$} 
        \Indent
            
            \State \textbf{if} $stage == \text{'pending framing'}$
            \Indent
                \State \textbf{if} $clock.now-frameStart \leq tout_3$
                \Indent
                    \State $x \leftarrow secret$
                    \State compute $verReveal$
                    \State \textbf{if} $H(pk||secret) == framingCommit$ \textbf{and} $verReveal$ 
                    \Indent
                        \State pay $pk$ \$($FRAMING\_DEPOSIT + \ell$)
                        \Statex\hskip6em ($balance \leftarrow balance - \$\ell -\$FRAMING\_DEPOSIT$)
                        \State $stage \leftarrow \text{`abort'}$
                    \EndIndent
                \EndIndent
                \State \textbf{else}
                \Indent
                    \State $stage \leftarrow \text{`reveal'}$
                \EndIndent
            \EndIndent
        \EndIndent
        
 	\end{algorithmic}
\end{algorithm}

==> our_EVR_solution.tex <==
We give some background and then introduce our solution to the EVR problem.

\subsection{Eth-DKG}
Eth-DKG~\cite{} is a variant of the Join-Feldman Distributed Key Generation (DKG) protocol~\cite{}, that is suited to work on Ethereum. For a detailed description and analysis of Eth-DKG see \cite{}. In this work we will only mention its properties and use it as a black-box. 

\subsection{Our EVR source}
The \ascii{commit} and \ascii{reveal} protocols that we use are the DKG and the reconstruction protocols in Eth-DKG. We will denote these as \ascii{DKGcommit} and \ascii{DKGreveal}. The smart contract that we implement, denoted $\G$, is a service in $\Z$, namely it is an escrow account with an initial registration stage in which investors register.
After registration, $\G$ adheres to the EVR source smart contract stage structure, defined in \cref{}. 

In Fig.~\ref{fig:G_alg} we give the pseudo-code for $\G$.
\input{figures/EVRS_algorithm}
% \input{figures/EVRS_algorithm_1}

\subsubsection{The commit stage}
$\G.\ascii{commit}$ starts by setting two important parameters: (i) $P=n/3$ (line~\ref{}), the economic worth of the randomness; and (ii) $t=2n/3$ (line~\ref{}), the threshold for learning the secret.

\red{Then, $\G.\ascii{commit}$ runs a distributed protocol that samples a secret and shares it among the investors using a Secret Sharing (SS) primitive~\cite{}. SS, with parameters $n$ and $t$, enables splitting a secret into $n$ processes, such that any $\ge t+1$ of them can reconstruct the secret and no $\le t$ of them can extract any information on the secret. Specifically, protocols in the spirit of Joint-Feldman Distributed Key Generation (DKG)~\cite{FeldmanVSS,PedersenDKG,DKG,Gennaro_DKG_99} can be used.} %Or with a trusted dealer (who samples $x$ and stops participating after distributing the shares).
Although the original DKG solutions function correctly under a model with a threshold of Byzantine processes, they have been adapted to work in our model of rational participants~\cite{rational_thresold_cryptosystems, EthDKG} with a concrete implementation for it in Ethereum~\cite{Github_DKG_Ethereum}. In~\cite{rational_threshold_cryptosystems} work, the DKG protocol is given as a service over a blockchain, using an abstraction similar to $\Z$, \idit{where/and} users register by depositing $1$ coin in order to participate. The main difference between this variant and traditional DKG protocols is that this protocol can fail, in which case deposits are returned. However, failure only happens if some participant broke the protocol's rules. This participant is identified and does not get her deposit back.

Here, we use the DKG protocol as a black-box and run it among our $N$ investors, where investor $i$ is represented $a_i$ times. The protocol generates a secret $x$ and $n$ shares for it. Investor $i$ ends up with $a_i$ shares. Any $t+1$ shares (or more) can reconstruct $x$, while any $t$ shares (or less) reveal nothing about $x$. When the DKG run ends, $X$ is published on $\G$, as a commitment for $x$. \red{In \Cref{} the DKG takes place in line We assume that the DKG run does not fail.} 

Finally, the \ascii{commit} protocol ends by setting $\ell=n$. This is a framing reward that will be explained below.

\subsection{$\G.\ascii{reveal}$ and $\G.\ascii{frame}$}
While $\G.\ascii{frame}$ is not part of the EVR interface, it is a function that $\G$ implements in order to satisfy the EVR \red{properties/requirements}. The framing mechanism is a key innovation in our solution. It is key to ensuring secrecy, namely that $x$ remains secret so long as $cnd$ does not mature (as defined in \cref{def:single-shot-EVR}). 

Note that the incentive to break secrecy is evident -- any investor (or group of investors) that obtains $x$ before $cnd$ matures may make a substantial profit (of up to $P$ coins, by the correct-usage definition). Framing nullifies this incentive by allowing any user that knows $x$ before $cnd$ matures to publish it on $\G$'s account for a high reward of \red{$\ell=n$} coins (line~\ref{alg:G:framing_reward}). These coins come from the investors' deposits, which are all confiscated in this case. The key property we utilize here is that in order to steal, at least one investor needs to locally reconstruct $x$. If this happens, that investor would have to make a decision -- to frame or to steal. As long as there is no investor who is better off stealing than framing, the framing mechanism is effective. It discourages investors from attempting to break secrecy as they realize that any one of them would frame if they had the possibility to do so.

Framing implies that $t+1$ (or more) accounts have reconstructed $x$ while it was forbidden to do so (note that from the commitment scheme being hiding, retrieving $x$ otherwise is impossible) and can be seen as a collective punishment \red{against the investors}. The framer who ``betrays'' the collusion is rewarded for her actions. If multiple framers attempt to frame, $\G$ rewards the one with the minimal id.    

If framing happens, $\G$ aborts, that is, it enters a state in which all calls to its functions return `fail' (specifically a call to the \ascii{reveal} function). 

If framing does not occur and $\G.\ascii{reveal}$ is invoked when $cnd$ matures, the investors may reconstruct $x$ \idit{(explain that they have a protocol (black-box?) that does this and creates a revealing transaction for them)} and get their deposits back in return for publishing it. If they do not publish $x$ in a timely manner, $\G$ aborts and all their deposits are confiscated (line~\ref{alg:G:secret_not_revealed}). Note that at least $n-t$ accounts must refrain from participating in order to prevent the publication of $x$.
 



==> proofs/Theorem_CPNE.tex <==
\begin{theorem} \label{Theorem:CPNE}
$s^*$ is a CPNE in $\game$.
\end{theorem}

\begin{proof}
Consider a coalition $C$ that deviates from $s^*$ resulting in a strategy vector $s=(s_C,s^*_{-C})$. 

If $s\in S_-$, then let $j\in [N]$ be an investor for whom $u_j(s) < 0$. Surely, $j\in C$, as if $j$ does not engage in any side contracts (as in $s^*$), she cannot lose any of her external coins and is thus guaranteed a non-negative payoff. Thus, $j$ is a deviating investor who loses from the deviation.

It remains to consider $s\in S_+$. Consider two cases:
\begin{enumerate}
    \item $\emph{SEC}(s)$. From Lemma~\ref{Lemma:SNE_robustness_secrecy}, there exists an investor $i\in C$ such that $u_i(s^*) \ge u_i(s)$, that is, $i$ is a member of $C$ that is not better off due to the deviation.
    
    \item $\neg \emph{SEC}(s)$. From \Cref{Lemma:collusion_CPNE} either $s$ is not self-enforcing or there exists an investor $j\in C$ who is not better off due to the deviation.
\end{enumerate}

% It remains to consider $s\in S_1$. Consider three cases:
% \begin{enumerate}
%     \item If $T(s)$ then at least one investor has $t+1$ shares at the end of stage 1. Let $f\in [N]$ be the smallest id among investors with $t+1$ shares or more at the end of stage 1. Because $T(s) \rightarrow \neg F(s)$ and in $s^*$ $f$ frames, we get that $f\in C$. By Lemma~\ref{lemma:dominant_strategy}, $f$ can further deviate from $s_C$ by framing instead of stealing the jackpot, guaranteeing herself a higher payoff. This implies that $C$'s deviation is not self-enforcing. Note that $f$'s second deviation from $s_C$ to framing is unilateral, and therefore self-enforcing.
    
%     \item If $F(s)$ then by Lemma~\ref{Lemma:base-game_SNE} at least one member of $C$ is not better off due to the deviation.
    
%     \item Finally, if $\neg T(s)$ and $\neg F(s)$ then from Lemma~\ref{Lemma:robustness_secrecy_sub-game} we know that there exists an investor $i\in C$ such that $u_i(s^*) \ge u_i(s)$, that is, $i$ is a member of $C$ that is not better off due to the deviation.
% \end{enumerate}
We have shown that any possible deviation of a coalition $C\subseteq [N]$ from $s^*$ is either not self-enforcing or includes a member that is not better off. Hence, $s^*$ is a CPNE in $\game$ as required.
\end{proof}

==> trash/EVRS_primitive.tex <==
In this section we define the problem that we set to solve in this work through the \emph{Economically Viable Randomness} (EVR) primitive. Loosely speaking, the EVR primitive can be seen as an economic extension of a distributed commit-reveal scheme~\cite{}, where the committed value is sampled uniformly at random from some domain. The random value has economic implications in the sense that it determines who makes a profit and who loses. EVR is to be used by a consumer application that requires random bits for its operation. Think of the consumer as a lottery, and of EVR as the randomness that determines the winner. In \Cref{sec:commitment_schemes} we review commitment schemes and in \Cref{sec:EVRS_single_shot} we define a simplified single-shot EVR. The full-fledged multi-shot primitive is given only at the end of the paper~\ref{}, before we describe our prototype implementation~\ref{}.

\subsection{Background -- Commitment Schemes} \label{sec:commitment_schemes}
A commitment scheme~\cite{} is a pair of efficient algorithms $(\ascii{com}, \ascii{ver})$ that allows a committer to bind herself to a private bit string $x$ by publishing a corresponding commitment $X=\ascii{com}(x)$. The algorithm \ascii{com} is \emph{binding}, preventing the committer from ``changing her mind'' after the fact and convincing a verifier that she committed to a different value. The commitment is \emph{hiding}, preventing learning anything about $x$ from $X$. The Boolean function $\ascii{ver}(x',X')$ is used in order to check whether a candidate value, $x'$, is consistent with a given commitment, $X'$.
% As an aside, we note that a commitment scheme can be generalized, committing to a collection of bit strings, as for example done in PoW schemes, where...

\red{An example of a (homomorphic) commitment scheme is the Pedersen commitment scheme~\cite{ped_commitment}.} \idit{Why this scheme is good for us? Any specific properties that are good for us? If we can cite a few different commitment schemes that all of them are suitable for us it would be better.}

\idit{Shouldn't there be background about commit-reveal schemes?}

\subsection{Single-Shot EVR Interface and Guarantees} \label{sec:EVRS_single_shot}
The EVR primitive executes in two phases: a \ascii{commit} phase and a \ascii{reveal} phase. The \ascii{commit} phase produces and publishes (in $\Z$) a commitment $X$ to a secret bit string $x$, sampled uniformly at random. Alongside $X$, it also publishes a value $B$, which, loosely speaking, is the \emph{\red{economic worth}} of the commitment, in $\Z$ coins.
The \ascii{reveal} phase publishes the secret $x$ when it is safe do so.

We first define single-shot EVR, in which the commitment corresponds to a single random value. We will later extend it to multi-shot EVR, in which a single commitment corresponds to a sequence of random values. 

Consider a commitment scheme $(\ascii{com},\ascii{ver})$. Let $cnd$ be a verifiable condition in $\Z$ that matures at some point \red{($cnd$ indicates when it is safe to publish the random bits).}

An EVR exposes the following interface:
\begin{enumerate}
    \item A call $\ascii{commit}(cnd)$ either fails or passes within a predetermined time limit. In case it fails it returns `fail'. In case it passes it returns a pair $(B, X)$, where $X=\ascii{com}(x)$ is a commitment to a bit string $x$, sampled uniformly at random, and $B\in \mathbb{N}_0$ indicates an economic value (in $\Z$ coins). We refer to $X$ as the EVRS commitment, and to $x$ as the EVRS secret.
    
    %\red{OR: An invocation $\ascii{commit}(cnd)$ returns a pair $(B, X)$ within a predetermined time limit, where $X=\ascii{com}(x)$ is a commitment to a bit string $x$, sampled uniformly at random, and $B\in \mathbb{N}$ \red{(an amount of coins in $\Z$).} If however, the pair $(B, X)$ is not returned, $\ascii{commit}(cnd)$ aborts and returns `fail'.} 
    
    \item A call $\ascii{reveal}()$ either fails or passes within a predetermined time limit. In case it fails it returns `fail'. In case it passes it returns the value $x$ such that $\ascii{ver}(x,X)=True$.
    
    %\red{OR: An invocation $\ascii{reveal}()$ returns the value $x$ within a predetermined time limit, such that $\ascii{ver}(x,X)=True$. If however, $x$ is not returned, $\ascii{reveal}()$ aborts and returns `fail'.}
\end{enumerate}

\begin{definition}[Single-shot EVRS]
\label{definition:EVR}
An escrow account $\E$ in $\Z$ is a single-shot EVRS if it implements the EVRS interface such that the following properties hold:
\begin{enumerate}
    \item Non-triviality. A call $\E.\ascii{commit}(cnd)$ \red{(before $cnd$ matures)} passes. %\idit{Our solution guarantees Non-triviality? Maybe we can say we guarantee it in certain circumstances?}
    
    \item Secrecy. If $\E.\ascii{commit}(cnd)$ passes, then before $cnd$ matures no \red{user} obtains any information about the EVRS secret. 

    \item Robustness. If $\E.\ascii{commit}(cnd)$ passes, then after $cnd$ matures, a call $\E.\ascii{reveal}()$ passes and returns the secret.
\end{enumerate}
\end{definition}

When a consumer (for instance a lottery) wishes to use an EVRS it establishes an adequate condition $cnd$ (e.g., a time in the future), invokes $\ascii{commit}(cnd)$, and gets the pair $(B,X)$. Now the consumer has the randomness committed to and it can run whatever logic it needs to (e.g., sell lottery tickets). Then, when $cnd$ matures (in our example this would happen after the ticket sale closes), the consumer invokes $\ascii{reveal}()$, gets $x$ (such that $\ascii{ver}(x,X)=True$), and completes its logic according to the $x$ returned (in our example, the lottery pays the winner). The secret, $x$, has an economic value in the sense that whoever obtains $x$ before $cnd$ matures can steal the consumer's coins (in our lottery example, they can buy the winning ticket). Also, if the random bits fail to be revealed after $cnd$ matures (i.e., the call \ascii{reveal} returns `fail'), the consumer still needs to do something with its coins (for instance, the consumer can burn its coins, or in the lottery example, it can refund the tickets). The EVRS does not assume anything if it fails to provide $x$, and accounts for the worst case in which someone can gain all the consumer's coins in case of such a failure.

A consumer has a few restrictions it must respect in order for the EVRS to satisfy its properties, as we now define:
\begin{definition}[Correct usage of a single-shot EVRS]
\label{def:evrs-usage}
A correct consumer of an EVRS sets $cnd$ such that:
\begin{enumerate}[label=C\arabic*.,ref=C\arabic*]
    \item Less than $B$ coins can be gained from obtaining $x$ before $cnd$ matures. \label{def:evrs-usage:before_cnd}
    \item No coins can be gained from obtaining $x$ after $cnd$ matures. \label{def:evrs-usage:after_cnd}
\end{enumerate}

In addition, it restricts the value of the randomness as follows:
\begin{enumerate}[label=B\arabic*.,ref=B\arabic*]
    \item No coins can be gained from the failure of \ascii{commit}. \label{def:evrs-usage:commit}
    \item Less than $B$ coins can be gained from the failure of \ascii{reveal}. \label{def:evrs-usage:reveal}
\end{enumerate}
\end{definition}
\idit{We can say that we formalize these in the analysis...}

% \red{When we explain what ``can be gained from'' means, we need to take into account that knowing $x$ or failing \ascii{reveal} can give an advantage in expectancy, rather than sure profits...} \idit{It is complex... Expectancy on what sample space? Only the bits of $x$ of also the strategies of the others?}

% \sout{For a consumer to correctly use an EVRS it must set an appropriate $cnd$ (the first 2 items), and it must restrict the economic worth of the random process (the last 2 items). We use our running lottery example to elaborate.} 

Consider, for instance, our lottery example.
To make sure that nothing can be gained by failing \ascii{commit} (\ref{def:evrs-usage:commit}), the lottery opens the ticket sale after \ascii{commit} passes. To ensure that after $cnd$ matures, knowing the secret does not give users an advantage in winning coins (\ref{def:evrs-usage:after_cnd}), $cnd$ matures after the lottery ticket sale closes. Finally, by restricting the amount raised (from ticket sales) to $B$ coins, the lottery ensures that failing \ascii{reveal} or obtaining $x$ before $cnd$ matures is worth no more than $B$ coins (\ref{def:evrs-usage:reveal} and \ref{def:evrs-usage:before_cnd}). \sout{In more general terms, as long as the consumer maintains its total payouts under $B$ it satisfies these conditions.}




==> trash/EVRS_realization.tex <==
\red{Many solutions for the EVR primitive may be devised, in this section we give our solution.}

Generally speaking, our solution to the EVR primitive is a distributed \red{commit-reveal scheme / coin toss protocol} with deposits and penalties, that are managed by an \red{escrow service} $\G$ in $\Z$. In our model, we have assumed that $\G$'s registration phase is over. $\G$ implements the \ascii{commit} and \ascii{reveal} functions and satisfies the properties of an EVRS primitive under certain conditions. Our solution uses a distributed key generation protocol (DKG) as a black-box. \idit{What's the black-box's interface? $X \leftarrow DKG(n,t)$ and $ver(x,X)$?} In Fig.~\ref{fig:G_alg} we give the pseudo-code for $\G$.

\idit{Say here what the following subsections contain. Say that first we present one-shot and then we explain multi-shot...}

\red{Do we need to give a brief background on secret sharing and DKG?}

\input{figures/EVRS_algorithm}

\subsection{$\G.\ascii{commit}$}
\label{black_box}
$\G.\ascii{commit}$ is responsible to generate a secret (the random bits), commit to it, and distribute cryptographic shares for it among the registered investors.  

$\G.\ascii{commit}$ sets the economic worth of the EVRS, $B=n/3$, as defined in line~\ref{}. It also sets the threshold parameter $t=2n/3$ which is the bound to reconstruct the secret from its shares. 
%\Cref{alg:G:param_n,alg:G:param_t,alg:G:param_B,alg:G:black-box} determine $\G$'s parameters: $X$ is the commitment for the underlying secret $x$; $n$ is the number of accounts that registered and correspondingly, the number of shares generated for $x$; $B=\nicefrac{n}{3}$ is the economic worth of the commitment; and $t=\nicefrac{2n}{3}$ is the threshold parameter, namely $t+1$ of shares are required in order to reconstruct $x$. 

In \cref{alg:G:black-box}, the black-box DKG executes, and if successful, a secret $x$ is randomly sampled and distributed among the $n$ registered accounts, each account holding a single cryptographic share. Any $t+1$ such shares can be used to reconstruct $x$, whereas any collection of $t$ shares or less reveals nothing on $x$. In addition, a commitment $X=\ascii{com}(x)$ is calculated and published in $\G$. $\G.\ascii{commit}$ returns $X$ and $B$ (to the entity that called it). %and we assume that $x$ is obscure from any investor at this point. 
%The second stage (\Cref{alg:G:black-box}) of the \ascii{commit} function returns $X$ and $B$.   the secret $x$ is determined, where no investor knows its value. Every \red{registration} is entitled to a cryptographic share of the secret such that any $t+1$ shares can reconstruct the secret. The \ascii{commit} function returns $X=\ascii{com}(x)$ a commitment to the secret $x$, and $B$.

Share distribution can be implemented either with a trusted dealer (who samples $x$ and stops participating after distributing the shares) or with a protocol in the spirit of Joint-Feldman~\cite{FeldmanVSS,PedersenDKG,DKG,Gennaro_DKG_99}; in fact, a concrete  implementation in Ethereum is available here~\cite{Github_DKG_Ethereum,rational_thresold_cryptosystems}.

\subsection{$\G.\ascii{reveal}$ and $\G.\ascii{frame}$}
%By the return of $\G.\ascii{commit}$, any $t+1$ accounts (but not fewer) can reconstruct $x$ and at least $n-t$ accounts are necessary in order to prevent the publication of $x$. 
While $\G.\ascii{frame}$ is not part of the EVR interface, it is a function that $\G$ implements in order to satisfy the EVR properties. The framing mechanism is a key innovation in our solution and what ensures secrecy, namely that $x$ remains secret so long as $cnd$ has not yet matured. 

We note that the incentive to break secrecy is evident -- any investor (or group of investors) that obtains $x$ before $cnd$ matures may make a substantial profit (of up to $B$ coins) as the correct usage definition assumes. Framing nullifies this incentive by allowing any user that knows $x$ before $cnd$ matures to publish it on $\G$'s account for a high reward of \red{$\ell=n$} coins (line~\ref{alg:G:framing_reward}). These coins come from the investors' deposits, which are all confiscated in this case. The key property we utilize here is that in order to steal, at least one investor needs to locally reconstruct $x$. If this happens, that investor would have to make a decision -- to frame or to steal. As long as there is no investor that is better off stealing than framing, the framing mechanism does the job. It discourages investors from attempting to break secrecy as they realize that any one of them would frame if they had the possibility.

Framing implies that $t+1$ (or more) accounts have reconstructed $x$ while it was forbidden to do so (note that from the commitment scheme being hiding, retrieving $x$ otherwise is impossible) and thus punishment is deserved. The framer who ``betrays'' the collusion is rewarded for her actions. If multiple framers attempt to frame, $\G$ rewards that with the minimal id.    

If framing happens, $\G$ aborts, that is, it enters a state in which all calls to its functions return `fail' (specifically a call to the \ascii{reveal} function). If framing does not occur and $\G.\ascii{reveal}$ is invoked when $cnd$ matures, the investors may reconstruct $x$ \idit{(explain that they have a protocol (black-box?) that does this and creates a revealing transaction for them)} and get their deposits back in return for publishing it. If they do not publish $x$ in a timely manner, $\G$ aborts and all their deposits are confiscated (line~\ref{alg:G:secret_not_revealed}). Note that at least $n-t$ accounts must refrain from participating in order to prevent the publication of $x$.

\red{Move to prototype implementation section \idit{(you don't have to move it, you can simply point there by a reference)}:} On a practical note, we emphasize that in both framing and the final publication of $x$, we do not require revealing individual shares. This allows stirring much of the computational load off-chain and enables $\G$ to reach massive scale (in terms of the number of shares generated).


==> trash/EVR_definition.tex <==
In this section we define the problem that we set to solve in this work. Consider an application whose users are economically affected by the outcome of a random process, for example, a lottery that relies on randomly sampled numbers to select a winner that sweeps the jackpot. Given the economic implications, the random process is a target for manipulation. \red{We have hinted in the previous section that our solution, presented in \Cref{}, takes the form of a service in $\Z$ (i.e., a smart contract with an initial registration phase). Nonetheless, the formal description of the problem is given in general terms and is of importance for its own right. Different solutions can be devised, some of which might not require a service at all.}

The \emph{Economically Viable Randomness} (EVR) primitive provides randomness that can be used securely by a consumer. The primitive comprises an economically-aware randomness source -- upon a consumer's request, the source emits a random value that has an \sout{explicit} economic worth. The randomness source satisfies a set of requirements (defined below) that render the value it emits secure. There are some restrictions on its usage, formalized (below) as EVR correct-usage. Thus, a solution to the EVR primitive is a randomness source that when used correctly by a consumer satisfies the EVR requirements. 

We define the EVR \red{primitive} over $\Z$. $\Z$ provides trustworthy execution of (deterministic) code, and a way to transfer economic value (coins). 
% For simplicity and clarity of the exposition, we define here a single-shot EVR. The full-fledged multi-shot primitive deferred to \Cref{}, before we describe our prototype implementation.

An \emph{EVR source} is a pair of protocols, \ascii{commit} and \ascii{reveal}, and a Boolean verification algorithm \ascii{ver}. The \ascii{commit} protocol publishes a commitment $X$ that binds the EVR source to some $x\in \{0,1\}^k$. At this point, the random value is committed to and can no longer be changed. The commitment is \emph{hiding}, namely, no actor can guess any of $x$'s bits with probability higher than $\nicefrac{1}{2}$. The \ascii{commit} is economically-aware in the sense that it is responsible to set the \emph{\red{economic worth}} of the randomness, as an amount of coins. The \ascii{reveal} protocol runs at a later time, and publishes $x$ when it is safe to do so, according to a verifiable condition in $\Z$ that the consumer provides. The \ascii{ver}$(x,X)$ function can then be used by anyone to verify that $x$ indeed corresponds to $X$.

Generally, an EVR source produces a sequence of random values, one after the other. This is useful for consumers that proceed in multiple rounds and need a fresh random value for every round (e.g, card and die games). To keep the presentation clear and concise, during most of this work, we will discuss a single-shot version of the EVR source. Later, in \cref{} we will extend it to multi-shot EVR, in which a single commitment corresponds to a sequence of random values that are revealed in order.

The following definition describes the interface that a single-shot EVR source exposes and captures the requirements it must satisfy so that the randomness that it produces is safe to use.
\begin{definition}[Single-shot EVR source]
\label{def:single-shot-EVR}
An EVR source is a tuple $(\ascii{commit},\ascii{reveal},,\ascii{ver},\E)$, where:
\begin{enumerate}
    \item \ascii{commit} is a protocol. A successful run of \ascii{commit} produces a commitment, $X$.
    
    \item \ascii{reveal} is a protocol. It is tied to a specific run of \ascii{commit}, such that a successful run of \ascii{reveal} produces $x$, the value that corresponds to the commitment that the \ascii{commit} run produced.
    
    \item \ascii{ver} is a Boolean algorithm that ties the \ascii{commit} and \ascii{reveal} protocols. $\ascii{ver}(x',X')$ returns true if and only if the value $x'$ corresponds to the commitment $X'$. 
    
    \item $\E$ is a smart contract in $\Z$ that exposes the following interface:
    \begin{enumerate}
        \item A call $\E.\ascii{commit}(cnd,\red{tout})$, where $cnd$ is a verifiable condition in $\Z$ and $tout$ indicates a timeout length, initiates $\E$'s \emph{commit phase}. The \emph{commit phase} lasts $tout$ seconds in which a \ascii{commit} run takes place and must publish the commitment $X$ on $\E$.    triggers a run of the \ascii{commit} protocol and. It , either fails or passes \red{within a time limit of $tout$ seconds}. In case it fails it returns `fail'. In case it passes it returns a pair $(P, X)$, where $X$ is a commitment to a bit string $x$, whose bits were sampled uniformly at random, and $P\in \mathbb{N}_0$ indicates an economic value (in $\Z$'s coins). We refer to $X$ as the commitment, and to $x$ as the secret.
        
        \item A call $\E.\ascii{reveal}()$ either fails or passes \red{within a time limit of $tout$ seconds}. In case it fails, it returns `fail'. In case it passes, it returns $x$ such that $\E.\ascii{ver}(x,X)=true$.
        
        \item A call $\E.\ascii{reveal}()$ either fails or passes \red{within a time limit of $tout$ seconds}. In case it fails, it returns `fail'. In case it passes, it returns $x$ such that $\E.\ascii{ver}(x,X)=true$.
\end{enumerate}

$\E$ satisfies the following requirements: %\sout{in $\Z$} is a single-shot EVR if it implements the randomness source interface such that the following properties hold:
\begin{enumerate}
    \item Non-triviality. A call $\E.\ascii{commit}(cnd)$ passes. %\idit{Our solution guarantees Non-triviality? Maybe we can say we guarantee it in certain circumstances?}
    
    \item Secrecy. If $\E.\ascii{commit}(cnd)$ passes, then before $cnd$ matures no user obtains any information about the secret. 

    \item Robustness. If $\E.\ascii{commit}(cnd)$ passes, then after $cnd$ matures, a call $\E.\ascii{reveal}()$ passes and returns the secret.
\end{enumerate}
\end{enumerate}
\end{definition}

\begin{remark}
Many types of cryptographic primitives can be adapted to adhere to the EVR's interface. Examples include protocols that rely on classical commitment schemes (as done in this work), for instance, Pedersen commitments~\cite{}. Protocols that rely on computational delay or time-lock puzzles can also work -- an input to a delay function~\cite{} or a VDF~\cite{} can serve as a commitment under certain conditions, or a PoW scheme can be used. Note that in some cases, a commitment might have multiple corresponding values, each of which could be the one revealed (as in PoW). 
\end{remark}

% \begin{remark}
% \sout{There are two major families of protocols that are suitable to anchor randomness sources. In the first family, protocols rely on commitment schemes, and in the second family, protocols rely on computational delay or time-lock puzzles.} 

% \sout{In the first case, $x$ is produced via a distributed protocol, such that every participant obtains only a cryptographic share of $x$ and no participant can learn anything about $x$. $X=\ascii{com}(x)$ on the other hand, is made available to all participants. In the second case, $x$ can be computed from $X$, but it takes time to compute and is thus secret from the time the first actor obtains $X$ and for the period of time that the computation takes.}
% \end{remark}

When a consumer (for instance a lottery) wishes to use an EVR source it establishes an adequate condition $cnd$ (e.g., a time in the future), invokes $\ascii{commit}(cnd)$, and gets the pair $(P,X)$. Now the consumer has the randomness committed to and can run whatever logic it needs to (e.g., sell lottery tickets). Then, when $cnd$ matures (in our example this would happen after the ticket sale closes), the consumer invokes $\ascii{reveal}()$, gets $x$ (such that $\ascii{ver}(x,X)=true$), and completes its logic according to the $x$ returned (in our example, the lottery pays the winner). The secret, $x$, has an economic value in the sense that whoever obtains $x$ before $cnd$ matures can steal the consumer's coins (in our lottery example, they can buy the winning ticket). Also, if the random bits fail to be revealed after $cnd$ matures (i.e., the call \ascii{reveal} returns `fail'), the consumer needs to decide what to do with its coins. For instance, the consumer can burn its coins, or in the lottery example, it can refund the tickets. The EVR source must account for the worst case in which someone can gain all the consumer's coins in case of such a failure.

A consumer has a few restrictions it must respect in order for the EVR source to satisfy its properties, as we now define:
\begin{definition}[Single-shot EVR correct-usage]
\label{def:evrs-usage}
A correct consumer of an EVR source sets a verifiable condition, $cnd$, that matures at some point. $cnd$ must satisfy the following conditions:
\begin{enumerate}[label=C\arabic*.,ref=C\arabic*]
    \item Less than $P$ coins can be gained from obtaining $x$ before $cnd$ matures. \label{def:evrs-usage:before_cnd}
    \item No coins can be gained from obtaining $x$ after $cnd$ matures. \label{def:evrs-usage:after_cnd}
\end{enumerate}

In addition, when it calls the source's protocols it must make sure that:
\begin{enumerate}[label=F\arabic*.,ref=F\arabic*]
    \item No coins can be gained from the failure of \ascii{commit}. \label{def:evrs-usage:commit}
    \item Less than $P$ coins can be gained from the failure of \ascii{reveal}. \label{def:evrs-usage:reveal}
\end{enumerate}
\end{definition}
These restrictions are reflected in the utility functions of the game we define in \Cref{}. For now, we continue with the lottery example to give intuition as how correct-usage is to be enforced by a consumer of an EVR source. To make sure that nothing can be gained by failing \ascii{commit} (\ref{def:evrs-usage:commit}), the lottery opens the ticket sale after \ascii{commit} passes. To ensure that after $cnd$ matures, knowing the secret does not give users an advantage in winning the jackpot (\ref{def:evrs-usage:after_cnd}), $cnd$ matures after the ticket sale closes. Finally, by restricting the amount raised (from ticket sales) to $P$ coins, the lottery ensures that failing \ascii{reveal} or obtaining $x$ before $cnd$ matures is worth no more than $P$ coins (\ref{def:evrs-usage:reveal} and \ref{def:evrs-usage:before_cnd}). Note that whenever the consumer maintains its total payouts under $P$ it satisfies the two latter conditions.

% \red{When we explain what ``can be gained from'' means, we need to take into account that knowing $x$ or failing \ascii{reveal} can give an advantage in expectancy, rather than sure profits...} \idit{It is complex... Expectancy on what sample space? Only the bits of $x$ of also the strategies of the others?}

% \sout{For a consumer to correctly use an EVRS it must set an appropriate $cnd$ (the first 2 items), and it must restrict the economic worth of the random process (the last 2 items). We use our running lottery example to elaborate.} 



==> trash/EVR_ideal_sources.tex <==
Consider an application whose users are economically affected by the outcome of a random process, for example, a lottery. Given its economic implications, the random process is a likely target for manipulation. In this section we define a randomness source that can safely provide the random bits in such circumstances. Our goal in the rest of the paper is to realize such a source. 

As a starting point we assume that the application is implemented as a smart contract \red{in} $\Z$. In this way, the application's deterministic logic is guarantees to execute as specified. However, as $\Z$'s State Machine is deterministic, the randomness generation cannot happen purely on-chain. Whenever the application needs a random value it triggers the randomness source. This source must have an off-chain component, where the sampling actually happens. Then, the random value is published on $\Z$ for the application to use.

In many games of chance (applications that require randomness), there is a stage where gamblers/players make choices/bets not knowing what the random value is going to be, and then the random value is revealed and certain gamblers make a profit and other lose. To adjust this to $\Z$'s terms, we let the application set a verifiable condition in $\Z$, \emph{cnd}, that matures at some point. For the application to work as intended, the randomness must remain completely obscure until \emph{cnd} matures, and then it needs to be revealed in the clear.

In \Cref{ssec:ideal} we define an ideal on-chain randomness source that could be used by applications in this manner. While an ideal source might be hard to realize, we define in \Cref{ssec:EVR} an economically viable randomness source, which defines restrictions on the economic value of the randomness. An application that adheres to these restrictions can use an EVR source instead of an ideal one.

%We refer to the application as the \emph{consumer} of the randomness, which is provided by a \emph{randomness source}.

\subsection{Ideal Source}
\label{ssec:ideal}
A \emph{single-shot
on-chain randomness source} consists of a pair of 
protocols,   \ascii{commit}
and \ascii{reveal}, and a smart contract  $\E$ in $\Z$, as follows:
\begin{enumerate}
    \item %A \ascii{commit} protocol. 
    A (successful) run of \ascii{commit} produces a commitment, $X$, to a random sample $x$ and publishes $X$ {on $\E$}. Note that a \ascii{commit} run has an off-chain component. 
    
    \item %A \ascii{reveal} protocol. 
    Following a \ascii{commit} run, a (successful) run of \ascii{reveal} reconstructs the value committed to, $x$, and publishes it on $\E$. The \ascii{commit} and \ascii{reveal} protocols are tied together through a well-known Boolean verification function $\ascii{ver}(x,X)$. For every $X$ and for every $x_1 \ne x_2$ either $\ascii{ver}(x_1,X)=\emph{false}$ or $\ascii{ver}(x_2,X)=\emph{false}$.
    
    \item $\E$ serves as an interface to the two protocols,  exposing the following API:
    \begin{enumerate}
        \item A function \emph{comTrigger}(\emph{cnd}) called by the application that triggers a \ascii{commit} run, where \emph{cnd} is a verifiable condition in $\Z$, determined by the application, that eventually matures. Once \emph{cnd} matures a \ascii{reveal} run begins.
    
        \item Two Boolean variables, \emph{verCom} and \emph{verRev}, that indicate whether the \ascii{commit} and \ascii{reveal} runs (resp.) have succeeded. \emph{verRev} is updated via a straightforward check with the function \ascii{ver}. \emph{verCom} is protocol-specific.
    
        \item Two timeout constants, $t_{\text{com}}$ and $t_{\text{rev}}$, that dictate the maximum time that the \ascii{commit} and \ascii{reveal} runs (resp.) can take. In case one of the runs does not complete in a timely manner, $\E$ sets the appropriate Boolean variable to \emph{false}.
    \end{enumerate}
\end{enumerate}

An \emph{ideal single-shot on-chain randomness source} is randomness source that is always safe to use by an application, as it satisfies the following core properties:
\begin{description}
    \item[Non-triviality] If $\E$.\emph{comTrigger}(\emph{cnd}) is called, then $\E.\emph{verCom}$ turns \emph{true}.
    
    \item[Secrecy] If $\E.$\emph{verCom} turns \emph{true}, then as long as \emph{cnd} does not mature, no user obtains $x$. 
    The secrecy is \emph{hiding} if no user obtains \emph{any} information about $x$.

    \item[Robustness] If $\E.\emph{verCom}$ turns \emph{true}, then after \emph{cnd} matures $\E.\emph{verRev}$ also turns \emph{true}.
    
    % \item[Unbiasability] If $\E.\emph{verCom}$ turns \emph{true}, then there a single 
\end{description}
Secrecy implies that it is computationally infeasible to learn $x$ from $X$ (and from participating in the \ascii{commit}'s run). Hiding secrecy is stronger and implies that $X$ is a cryptographic commitment in the sense that it is hiding (loosely speaking, if no one can infer any of $x$'s bits with probability greater than $\nicefrac{1}{2}$, it implies that $x$ is a random bit-string). The Boolean function \ascii{ver} implies that $X$ binds the source to a specific random value. So, once $X$ is published on $\E$, $x$ is determined and can no longer change (no other value would be accepted as the ``randomness'').

An ideal source (that satisfies hiding secrecy) is safe to use because it enables the application to run as intended. Intuitively, if the source does not satisfy these properties, then there are two opportunities for users to ``game the system''. First, obtaining any information about the secret before \emph{cnd} matures might give a user an advantage relative to what the application has intended, e.g., in a lottery such a user could buy a winning ticket with higher probability relative to ignorant players. Second, preventing the secret from being published after \emph{cnd} matures opens opportunities to profit from the application's fallback distribution, which is how the application spends its coins if $x$ is not published in a timely manner, e.g., a refund to the gamblers. An ideal source eliminates both these risks.

\begin{remark}
Generally, a randomness source produces a sequence of random values, one after the other. This is useful for applications that proceed in multiple rounds and need a fresh random value for every round (e.g., card and die games). To keep the presentation concise, during most of this work, we discuss a single-shot version of the EVR source. Later, in \Cref{sec:multi_shot_EVRS}, we extend it to multi-shot EVR, in which a single commitment corresponds to a sequence of random values that are revealed in order.
\end{remark}

\subsection{EVR Source}\label{ssec:EVR}
We are now ready to define a \emph{single-shot EVR source} that can be used in lieu of an ideal one in an economic environment. An EVR source is a randomness source, but it satisfies the core properties only provided that the application satisfies the economic restrictions laid out in \Cref{def:evrs-usage} below.

In order to define the economic conditions, we need to quantify the profits that can be gained by ``gaming the system'' and causing the EVR source to deviate from the ideal functionality. 
We say that a profit is \emph{illicit} if it is gained by breaking any of the ideal source's properties (on top of whatever legitimate profit is gained by using an ideal EVR source). 

The following economic restrictions on the application bound the illicit profit that an EVR source can sustain. As long as the application makes sure that no more illicit profit can be made, an EVR provides ideal-like randomness. $\E$ evaluates the bound on the illicit profit (possibly depending on certain aspects of the \ascii{commit} run) and publishes it in a variable we denote by $P$. A straightforward way for an application to bound the illicit profit to $P\ge 0$ coins is by limiting its total payouts to $P$.

\begin{definition}[Single-shot EVR correct-usage]
\label{def:evrs-usage}
An application correctly uses an EVR source if it satisfies the following conditions:
\begin{enumerate}[label=CU\arabic*.,ref=CU\arabic*]
    \item If non-triviality breaks, no user gains illicit profit. \label{def:evrs-usage:commit}
    
    \item If robustness breaks, the total illicit profit gained by all users is less than $P$. \label{def:evrs-usage:reveal}
    
    \item If secrecy breaks, the total illicit profit gained by all users is less than $P$. \label{def:evrs-usage:before_cnd}
    
    \item If secrecy and robustness are preserved, no user gains illicit profit. \label{def:evrs-usage:after_cnd}
\end{enumerate}
\end{definition}
These restrictions are reflected in the utility functions of the game we define in \Cref{sec:game-def}.

We next exemplify the interplay between the application and the EVR source and show that the correct-usage restrictions are feasible. When an application, for instance, a lottery, wishes to use an EVR source, it establishes an adequate condition \emph{cnd} (e.g., a time after ticket sales will close) and calls $\E$.\ascii{comTrigger}(\emph{cnd}). Once the pair $(P,X)$ is published on $\E$, the application has the randomness committed to and can run its logic, e.g., sell lottery tickets to gamblers. Then, when \emph{cnd} matures, the application needs $x$ (that corresponds to $X$) in order to complete its logic (in our example, determine the winning lottery tickets) and make payouts to winners.

If $x$ is not published in a timely manner, then the application uses some fallback rule to determine who gets its coins. This might be, but is not necessarily, a straightforward refund to the gamblers. %The EVR primitive does not restrict the application in any way in regards to this fallback distribution. In order for the consumer to offer good user experience / be competitive with centralized counterparts it is expected to reassure its users that in case of failure it would refund their tickets.
In contrast, if $X$ is not published, then \ref{def:evrs-usage:commit} dictates that no illicit profit can be made. This implies that the application cannot make any payouts (and particularly no refunds) in this case. Note that in order to be trusted by users, a dApp will want to refund gamblers in case of failure. Thus, to comply with \ref{def:evrs-usage:commit}, the application should start collecting coins from gamblers only after \ascii{commit}. In the lottery example, this means that ticket sales begin after the \ascii{commit} run completes. 

% \sout{To illustrate this, consider the lottery example. If, for instance, the ticket sale precedes \ascii{comTrigger}, then an attacker holding a specific set of lottery tickets that are not winners can make an illicit profit by failing the \ascii{commit} run and getting a refund on their tickets. So, to comply with \ref{def:evrs-usage:commit} the lottery begins selling tickets only after the \ascii{commit} run is complete.}
% \red{An EVR source does not want to impose on applications a state in which they have already raised coins from gamblers but cannot offer a refund for these coins. it does not have to be in such a state and \ref{def:evrs-usage:commit} stands.} 

To comply with \ref{def:evrs-usage:reveal} and \ref{def:evrs-usage:before_cnd} the application needs to maintain its total payouts under $P$. That is, $P$ bounds the jackpot that can be played for (in our lottery example, as long as the lottery raises less than $P$ coins from ticket sales, it adheres to these restrictions).  

Note that we use secrecy rather than hiding secrecy in \ref{def:evrs-usage:after_cnd}. This means that even if hiding secrecy breaks, the application still needs to make sure that there is no way to make an illicit profit. Put differently, the application must make sure that a gambler with partial information about $x$ (before \emph{cnd} matures) does not gain an advantage relative to gamblers with no information about $x$. To ensure this, $x$ must be used by the application carefully. In our example, if say half of $x$'s bits can be learned by a sophisticated player and the lottery's decision rule is $\min_{tickets}\{\text{XOR}(x,ticket)\}$, then that player has a significant advantage over other players. However, if the decision rule is $\min_{tickets}\{\text{hash}(x,ticket)\}$, then having partial information about $x$ does not help.

To comply with \ref{def:evrs-usage:after_cnd}, the application has to worry about one last pitfall. Investors might cooperate through a multi-party computation (MPC)~\cite{Yao-2PC,Yao-MPC,GMW-MPC,Ben-or_MPC1,Chaum-MPC,Rabin-MPC,Beaver-MPC,Canetti-MPC1,Canetti-MPC2} protocol that ensures the privacy of each investor's input (i.e., her shares), keeps all steps of the computations obscure, and finally outputs a winning ticket. In this way none of the investors actually learns $x$, but they still manage to infer a winning ticket (from which learning $x$ might still be hard). To circumvent this issue, the application must choose a decision rule that is ``MPC resistant'', namely that is slow to compute via MPC. %(Most decision rules should be fine, even in the best scenario, where there are two participating processes and they are both honest. A more formal analysis of this point is left for future work.) 
\red{(Currently, \cite{Efficient-MPC} presented one of the most efficient methods to compute general MPCs. There, a SHA-256 (that is also available in Ethereum smart contracts) 7-party computation, implemented as a Boolean circuit with $\approx $22,000 AND gates \cite{hash_gates}, takes about 20 seconds (over a fast LAN). However, it takes 7 orders of magnitude less to compute the same hash function on the same machine \cite{sha256_intel_xeon_computer}.}
%\sout{Therefore, 1 second long of sequential hashing would take almost 4 months to run in such an MPC.})

==> trash/EVR_primitive_lean.tex <==
In this section we define the problem that we set to solve in this work. Consider an application whose users are economically affected by the outcome of a random process, for example, a lottery. Given its economic implications, the random process is a likely target for manipulation. The \emph{Economically Viable Randomness} (EVR) primitive defines a source of randomness that can be safely used in such settings.

EVR is formalized as an interplay between two abstract entities -- the \emph{consumer} and the \emph{EVR source}. The consumer needs random values, and it triggers the EVR source to provide that randomness. In \Cref{sec:EVR_source} we formalize the guarantees of an EVR source, and in \Cref{sec:consumer_correct_usage} we define a number of requirements that the consumer must comply with in order to \sout{render the randomness provided by the EVR source safe to use by the consumer} enable/facilitate the EVR source to provide safe randomness.

\subsection{EVR Source} \label{sec:EVR_source}
\red{Maybe to intro: The EVR primitive uses $\Z$ as a means to decentralize the randomness generation process. However, randomness generation cannot happen purely on-chain because $\Z$'s State Machine is deterministic. Thus, any randomness source must have an off-chain component, where the sampling actually happens. Then, the random value is published on and verified by $\Z$.} 

An \emph{EVR source} is a pair of (off-chain) protocols, \ascii{commit} and \ascii{reveal} associated with a Boolean verification function $\ascii{ver}(x,X)$ such that for every $X$ and for every $x_1 \ne x_2$ either $\ascii{ver}(x_1,X)=\emph{false}$ or $\ascii{ver}(x_2,X)=\emph{false}$. The third element of an EVR source is a smart contact $\E$ on $\Z$ that verifies that runs of the two protocols complete successfully. $\E$ is an honest entity that is guaranteed to follow its instructions, and thus it is $\E$ that ascertains whether runs of the protocol succeed or fail. $\E$ acts as the source-of-truth to all users regarding the source's outcome.

$\E$ exposes a specific interface that ties it together with the two protocols. The interface includes:
\begin{enumerate}
    \item A function $\emph{comTrigger}(\emph{cnd})$ called by the consumer that triggers a \ascii{commit} run. \emph{cnd} is a verifiable condition, determined by the consumer, that is stored on $\E$'s state. Once this condition matures it triggers a \ascii{reveal} run.  
    
    \item Two Boolean variables, \emph{verCom} and \emph{verRev}, that indicate whether the \ascii{commit} and \ascii{reveal} runs (resp.) succeed or fail.
    
    \item Two timeout constants, $t_{com}$ and $t_{rev}$, that dictate the maximum time that the \ascii{commit} and \ascii{reveal} runs (resp.) can take. In case one of the runs does not complete in a timely manner, $\E$ sets the appropriate Boolean variable to \emph{false}.
\end{enumerate}

A run of the \ascii{commit} protocol produces a weak notion of commitment, $X$, and publishes it on $\E$'s state. The commitment \emph{binds} the EVR source to some random value $x$. Once $X$ is published, $x$ is determined and can no longer change, although it is not yet publicly known. Particularly, it is computationally infeasible to learn $x$ from the commitment (and from participating in the \ascii{commit}'s run). We note that $X$ is not necessarily hiding, i.e., it might leak some information about $x$. 
%(For our needs, we can think of $(x,X)$ as a secret and public key pair. Hardness of learning $x$ comes from some asymmetric function, as in typical key generation protocols.) 
\idit{(The possibility of extracting partial information about $x$ is discussed below.)}

$\E$ verifies that $X$ is a valid commitment \sout{(on-chain)}. (This verification is protocol-specific. For example, in some protocols, $X$ needs to correspond to private data that the \ascii{commit} run produces.) Given a run of the \ascii{commit} protocol committing to $x$, a subsequent run of the \ascii{reveal} protocol produces and publishes $x$ on $\E$'s state. $\E$ verifies that $x$ corresponds to $X$ (on-chain) using the Boolean function $\ascii{ver}(x,X)$.

\begin{remark}
Generally, an EVR source produces a sequence of random values, one after the other. This is useful for consumers that proceed in multiple rounds and need a fresh random value for every round (e.g., card and die games). To keep the presentation concise, during most of this work, we discuss a single-shot version of the EVR source. Later, in \Cref{sec:multi_shot_EVRS} we extend it to multi-shot EVR, in which a single commitment corresponds to a sequence of random values that are revealed in order.
\end{remark}

We now formalize the properties that render an EVR source safe to use by a consumer. We refer to an EVR source that satisfies these properties as an \emph{ideal source}. An \emph{ideal source} satisfies the following properties:
\begin{description}
    \item[Non-triviality] If $\E.\emph{comTrigger}(\emph{cnd})$ is called, then $\E.\emph{verCom}$ turns \emph{true}.
    
    \item[(Hiding) Secrecy] If $\E.\emph{verCom}$ turns \emph{true}, then as long as \emph{cnd} does not mature, no user obtains $x$. 
    (Moreover, no user obtains \emph{any} information about $x$.) 

    \item[Robustness] If $\E.\emph{verCom}$ turns \emph{true}, then $\E.\emph{verRev}$ also turns \emph{true}.
    
    % \item[Unbiasability] If $\E.\emph{verCom}$ turns \emph{true}, then
\end{description}

Our work implements an EVR source that can be used in lieu of an ideal one in an economic environment, provided that the consumer satisfies the economic restrictions laid out in \Cref{sec:consumer_correct_usage} below.

\subsection{Correct-Usage of an EVR Source} \label{sec:consumer_correct_usage}
In order to define the economic conditions for using our EVR source, we need to quantify the profits that can be gained by ``gaming the system'' and causing the EVR source to deviate from the ideal functionality. 
We say that a profit is \emph{illicit} if it is gained by breaking any of the ideal source's properties (on top of whatever legitimate profit is gained by using an ideal EVR source). 

The following economic restrictions, that apply to the consumer, indicate how much illicit profit can an EVR source ``endure''. As long as the consumer makes sure that no more illicit profit can be made, an EVR source is to provide ideal-like randomness. $\E$ evaluates the bound on the illicit profit (possibly depending on certain aspects of the \ascii{commit} run) in a variable we denote by $P$.

\begin{definition}[Single-shot EVR correct-usage]
\label{def:evrs-usage}
A correct consumer of an EVR source sets a verifiable condition, \emph{cnd}, that matures at some point, and satisfies the following conditions:
\begin{enumerate}[label=CU\arabic*.,ref=CU\arabic*]
    \item If non-triviality breaks, no user gains illicit profit. \label{def:evrs-usage:commit}
    
    \item If robustness breaks, the total illicit profit gained by all users less than $P$. \label{def:evrs-usage:reveal}
    
    \item If secrecy breaks, the total illicit profit gained by all users is less than $P$. \label{def:evrs-usage:before_cnd}
    
    \item If secrecy and robustness are preserved, no user gains illicit profit. \label{def:evrs-usage:after_cnd}
\end{enumerate}
\end{definition}
\red{We emphasize that we talk about secrecy here and not about hiding secrecy.}
% There are 3 types of necessary explanations here: (i) That these restrictions are feasible to comply with. (ii) That users can check that they are indeed respected. (iii) The motivation behind these restrictions and why we have them. We mostly focus on (i) here. (ii) is trivial. We show (iii) in the analysis where we point to where these restrictions are used in the proofs.

These restrictions are reflected in the utility functions of the game we define in \Cref{sec:game-def}. To clarify the interplay between the consumer and the EVR source, and to show that the correct-usage restrictions are reasonable, we put it all together.

When a consumer (for instance, a lottery) wishes to use an EVR source, it establishes an adequate condition $cnd$ (e.g., a time in the future) and calls $\E.\ascii{comTrigger}(cnd)$. Once the pair $(P,X)$ is published on $\E$, the consumer has the randomness committed to and can run whatever logic it needs (e.g., sell lottery tickets to gamblers). Then, when $cnd$ matures, the consumer needs $x$ (that corresponds to $X$), in order to complete its logic (in our example, determine the winning lottery tickets) and make payouts to winners. 

If $x$ is not published in a timely manner, then the consumer uses some fallback rule to determine who gets its coins (this might be, but is not necessarily, a refund to the gamblers). The EVR primitive does not restrict the consumer in any way in regards to this fallback distribution. %In order for the consumer to offer good user experience / be competitive with centralized counterparts it is expected to reassure its users that in case of failure it would refund their tickets.

\Cref{def:evrs-usage:commit} dictates that if $X$ is not published after the call $\E.\ascii{comTrigger}(cnd)$ then no illicit profit can be made. This implies that the consumer cannot make any payouts (and particularly no refunds) in this case. If the first thing that the consumer does is trigger the \ascii{commit} run, then no one can make any illicit profit from failing it. (To illustrate this point, consider the lottery example. If, for instance, the ticket sale precedes \ascii{comTrigger}, then an attacker holding a specific set of lottery tickets that are not winners would have made an illicit profit if the \ascii{commit} run failed and they got a refund on their tickets.)

To comply with \Cref{def:evrs-usage:reveal} and \Cref{def:evrs-usage:before_cnd} the consumer needs to maintain its total payouts under $P$. That is, $P$ bounds the jackpot that can be played for (in our lottery example, as long as the lottery raises less than $P$ coins from ticket sales, it adheres to these restrictions).  

To comply with \Cref{def:evrs-usage:after_cnd}, the consumer must make sure that: (i) there is not a way to infer a winning ticket without actually having $x$ (recall that an EVR source satisfies secrecy and not hiding secrecy), and (ii) obtaining $x$ after $cnd$ matures cannot result in illicit profits. The second item is straightforward (in our example, by closing the ticket sale before $cnd$ matures, the lottery makes sure that obtaining $x$ after $cnd$ matures is too late to make illicit profit). To comply with the first item, there are two further pitfalls.

First, a sophisticated user that can extract partial information about $x$ before $cnd$ matures (recall that $X$ is not a strictly hiding commitment) might permit to gain an unfair advantage in the lottery. To combat this issue, the way $x$ is used by the consumer to infer winners must be done carefully. (In our example, if say $20$ of $x$'s bits can be learnt by a sophisticated player and the lottery's decision rule is $min_{tickets}\{XOR(x,ticket)\}$, then that player has a significant advantage over simple players. However, if the decision rule is $min_{tickets}\{Hash(x,ticket)\}$ then having partial information about $x$ does not help. A further analysis into this issue is left for future work.)

Second, investors might cooperate such that together they provide $t+1$ shares (which suffices to reconstruct $x$), but within a multi-party computation (MPC)~\cite{} protocol that ensures the privacy of each investor's input (i.e., her shares) and outputs a winning ticket. The MPC ``goes through'' $x$ to compute the winning ticket, but in such a way that $x$ is never revealed to any of the investors. \red{MPCs are generally not practical to run, even in the best scenario, where there are two participating processes and they are both honest. They are theoretically possible for any function, but not necessarily practical~\cite{}. The lottery must make sure that its decision rule is not vulnerable to such an attack. Also, what does the MPC reveal about steps in the computation? If $x$ might be computed at some point, maybe it cannot be kept obscure from the participants? We need to verify this point.}

% \begin{remark}
% \red{Many types of cryptographic primitives can be adapted to adhere to the EVR's \red{structure/interface}. Examples include protocols that rely on classical commitment schemes (as done in \sout{this work} \idit{--put a citation or a reference to a section}), for instance, Pedersen commitments~\cite{}. Protocols that rely on computational delay or time-lock puzzles can also work -- an input to a delay function~\cite{} or a VDF~\cite{} can serve as a commitment under certain conditions, or a PoW scheme can be used. Note that in some cases, a commitment might have multiple corresponding values, each of which could be the one revealed (as in PoW).}
% \end{remark}

==> trash/EVR_primitive_new.tex <==
In this section we define the problem that we set to solve in this work. Consider an application whose users are economically affected by the outcome of a random process, for example, a lottery. Given its economic implications, the random process is a likely target for manipulation. The \emph{Economically Viable Randomness} (EVR) primitive defines a source of randomness that can be safely used in such settings.

EVR is formalized as an interplay between two abstract entities -- the \emph{consumer} and the \emph{EVR source}. The consumer needs random values, and it triggers the EVR source to provide that randomness. In \Cref{sec:EVR_source} we formalize the guarantees of an EVR source, and in \Cref{sec:consumer_correct_usage} we define a number of requirements that the consumer must comply with in order to render the randomness provided by the EVR source safe to use by the consumer.

\subsection{EVR Source} \label{sec:EVR_source}

The EVR primitive uses $\Z$ as a means to decentralize the randomness generation process. However, randomness generation cannot happen purely on-chain because $\Z$'s State Machine is deterministic. Thus, any randomness source must have an off-chain component, where the sampling actually happens. Then, the random value is published on and verified by $\Z$. %The definition of an EVR source does not restrict the off-chain process, but only establishes the interaction between the off-chain logic and $\Z$. \avi{we need to explain what is on/off-chain}

% We take a moment to explain the term \emph{protocol} that we use oftentimes in this work. By and large, a protocol is a set of instructions that a set of processes follow. A protocol run has an initial configuration that determines the set of participating processes (this set might be open or closed, static or dynamic, etc.) and potentially other parameters. The processes follow the protocol's instructions by which they produce private and public data. A correct run of a protocol ends in such a way that the private data held by each process and the public data satisfy certain invariants. A run might not be correct since some processes might diverge from their instructions. 

% In this work we are interested in protocols that interact with a smart contract. Specifically, we focus on protocols that can be ``overseen'' by a smart contract. We think of the smart contract as an additional participant, but not just a regular one, a trustworthy one. The protocol's instructions are adjusted such that participants submit certain data to the contract and the contract verifies that a given run is correct. The contract instructions are guaranteed to be followed correctly. 

An \emph{EVR source} is a pair of (off-chain) protocols, \ascii{commit} and \ascii{reveal} associated with a Boolean verification function $\ascii{ver}(x,X)$, and a smart contract $\E$ that adheres to a specific structure and \red{oversees} runs of the two protocols. %\avi{To keep the presentation concise, during most of this work, we discuss a single-shot version of the EVR source which produces a single random value. In \Cref{} we extend it to the multi-shot case.} \avi{(maybe instead of the remark below)} 

A run of the \ascii{commit} protocol produces a commitment, $X$, and publishes it on $\E$'s state. The commitment \emph{binds} the EVR source to some random value $x$. Once $X$ is published, $x$ is determined and can no longer change, although it is not yet publicly known.
Moreover, it is computationally infeasible to learn $x$ from the commitment and from participating in the \ascii{commit}'s run. We note that $X$ is not necessarily hiding, i.e.,  it 
%(as in the sense of the hiding game), and 
might leak some information about $x$. 
%(For our needs, we can think of $(x,X)$ as a secret and public key pair. Hardness of learning $x$ comes from some asymmetric function, as in typical key generation protocols.) 
\idit{(The possibility of extracting partial information about $x$ is discussed below.)}

$\E$ verifies that $X$ is a valid commitment (on-chain). (This verification is protocol-specific. For example, in some protocols, $X$ needs to correspond to private data that the \ascii{commit} run produces.) Given a run of the \ascii{commit} protocol committing to $x$, a subsequent run of the \ascii{reveal} protocol produces and publishes $x$ on $\E$'s state. $\E$ verifies that $x$ corresponds to $X$ (on-chain) using the Boolean function $\ascii{ver}(x,X)$.

$\E$ triggers the run of each of the protocols and ensures that they complete correctly and in a timely manner. It tracks their states via two Boolean state variables, $\E.verCommit$ and $\E.verReveal$, which indicate whether the \ascii{commit} and \ascii{reveal} (resp.) protocols complete correctly. E.g., when $\E$ obtains $X$ and verifies that the data produced by the run is consistent, $\E.verCommit$ turns \emph{true}. 
% Similarly, $\E.verReveal$ is a Boolean variable that indicates whether the \ascii{reveal} run completes correctly. %A \ascii{reveal} run is tied to a previous \ascii{commit} run in that part of the \ascii{reveal}'s initial configuration is $X$, the commitment that the \ascii{commit} run produced. $\E.verReveal$ turns $true$ if $\E$ obtains the value that the \ascii{reveal} run produced, $x$, and it corresponds to $X$. 

\red{The interface between the protocols and the smart contract is given by two timeout constants, two Boolean variables that signal whether they complete successfully, and a function to trigger a \ascii{commit} run...}

On top of overseeing the \ascii{commit} and \ascii{reveal} protocols, $\E$ evaluates the \emph{economic worth} of the EVR's randomness in terms of $\Z$'s coins. This evaluation enables \red{us} to define quantitative restrictions that apply to the consumer and establish the conditions that let the EVR source provide secure randomness.
%This bound limits the economic implications that the consumer can attribute to the randomness.

\begin{remark}
Generally, an EVR source produces a sequence of random values, one after the other. This is useful for consumers that proceed in multiple rounds and need a fresh random value for every round (e.g., card and die games). To keep the presentation concise, during most of this work, we discuss a single-shot version of the EVR source. Later, in \Cref{sec:multi_shot_EVRS} we extend it to multi-shot EVR, in which a single commitment corresponds to a sequence of random values that are revealed in order.
\end{remark}

% The consumer, through $\E$, triggers \ascii{commit} to start running. Then, $\E$ makes sure that the \ascii{commit} run publishes a commitment $X$ on-chain within a predetermined timeout. The commitment \emph{binds} the EVR source to some $x\in \{0,1\}^k$, and so, the random value is determined and can no longer change. The commitment is also \emph{hiding}, namely, no actor can guess any of $x$'s bits with probability higher than $\nicefrac{1}{2}$. The \ascii{commit} protocol is economically-aware in the sense that, on top of $X$, it also publishes the \emph{economic worth} of the randomness, as an amount of coins in $\Z$.

% The queue for \ascii{reveal} to start running is triggered when a verifiable condition in $\Z$, provided by the consumer, matures and declares that it is safe to publish $x$. Then, $\E$ makes sure that the \ascii{reveal} run publishes $x$ in a timely manner. Finally, $\E$ computes $\ascii{ver}(x,X)$ to verify that indeed $x$ corresponds to $X$.

We now formalize the definition of an EVR source.
\begin{definition}[Single-shot EVR source]\label{def:single-shot-EVR}
A single-shot EVR source consists of \ascii{commit} and \ascii{reveal} protocols and a smart contract $\E$ in $\Z$. 
$\E$'s variables include two (constant) timeout periods (in seconds), $tout_{com}$ and $tout_{rev}$; two Boolean variables $verCommit$ and $verReveal$\sout{; and an amount of coins in $\Z$, $P$}. $\E$'s functions include $\ascii{commitTrigger}(cnd)$, where $cnd$ is a verifiable condition in $\Z$. 
$\E$ advances in the following stages: 
% \begin{enumerate}
    % \idit{delete the enum...}
    
    % \item \sout{A \ascii{commit} protocol: A successful run of \ascii{commit} produces a commitment, $X$.}
    
    % \item \sout{A \ascii{reveal} protocol, that is tied to a specific run of \ascii{commit}: A successful run of \ascii{reveal} produces $x$, the value that corresponds to $X$.}
    
    % \item A function \ascii{ver} that links the \ascii{commit} and \ascii{reveal} protocols: $\ascii{ver}(x',X')$ returns $true$ if and only if the value $x'$ corresponds to the commitment $X'$. 
    
    % \item \sout{A smart contract} $\E$ \sout{in $\Z$ that} defines two timeout periods (in seconds), $tout_1$ and $tout_2$; a function $\ascii{commitTrigger}(cnd)$, where $cnd$ is a verifiable condition in $\Z$; and two Boolean variables $verCommit$ and $verReveal$, initiated to $false$. $\E$ advances in the following stages: 
    \begin{description}
        \item[Commit] A call $\E.\ascii{commitTrigger}(cnd)$ initiates the commit stage. The commit stage lasts at most $tout_{com}$ seconds, during which a \ascii{commit} run takes place (the run may invoke on- and off-chain computations). The commit stage ends successfully when $verCommit$ turns \emph{true} (which implies that a valid commitment produced by the \ascii{commit} run, $X$, is published on $\E$). However, if $tout_{com}$ seconds pass before this happens, then the stage fails. In the successful case, $\E$ designates a value $P\in \mathbb{N}$, which indicates the economic worth of the randomness (in $\Z$'s coins), and enters the pending stage. In case of failure, $\E$ enters the abort stage.
        
        \item[Pending] The pending stage lasts until $cnd$ matures, and then $\E$ enters the reveal stage.
        
        \item[Reveal] The reveal stage ends at most $tout_{rev}$ seconds after $cnd$ matures. During this time, a \ascii{reveal} run takes place (the run may invoke on- and off-chain computations). The reveal stage ends successfully when $verReveal$ turns \emph{true} (which implies that the value produced by the \ascii{reveal} run, $x$, is published on $\E$, and corresponds to $X$). However, if $tout_{rev}$ seconds pass before this happens, then the stage fails. In the successful case, $\E$ enters the final stage, and in case of failure, it enters the abort stage.
        
        \item[Final] The final stage indicates that the EVR source has completed successfully.
        
        \item[Abort] The abort stage indicates that the EVR source has failed. In this stage, any future call to any of $\E$'s functions fails.
\end{description}

An \emph{ideal EVR source} $\E$ satisfies the following properties: 
%\sout{in $\Z$} is a single-shot EVR if it implements the randomness source interface such that the following properties hold:
\begin{description}
    \item[Non-triviality] The commit stage ends successfully. %\idit{Our solution guarantees Non-triviality? Maybe we can say we guarantee it in certain circumstances?}
    
    \item[(Hiding) Secrecy] If the commit stage ends successfully, then during the pending stage, no user obtains $x$. 
    Moreover, no user obtains \emph{any} information about $x$. 

    \item[Robustness] If the commit stage ends successfully, then $\E$ reaches the final stage.
\end{description}
% \end{enumerate}
\end{definition}

Our work implements an EVR source that can be used in lieu of an ideal one in an economic environment, provided that the consumer satisfies the economic restrictions laid out in \Cref{sec:consumer_correct_usage} below.

\idit{Consider moving this paragraph to the next subsection.}
In order to define the economic conditions for using our EVR source, we need to quantify the profits that can be gained by ``gaming the system'' and causing the EVR source to deviate from the ideal functionality. 
We say that a profit is \emph{illicit} if it is gained by breaking any of the ideal EVR's properties (on top of whatever legitimate profit is gained by using an ideal EVR source). 


\subsection{Correct-Usage of an EVR Source} \label{sec:consumer_correct_usage}
When a consumer (for instance, a lottery) wishes to use an EVR source, it establishes an adequate condition $cnd$ (e.g., a time in the future) and calls $\E.\ascii{commitTrigger}(cnd)$. Once the pair $(P,X)$ is published on $\E$, the consumer has the randomness committed to and can run whatever logic it needs (e.g., sell lottery tickets). Then, when $cnd$ matures \sout{(in our example, after the ticket sale closes)}, the consumer needs $x$ (that corresponds to $X$), in order to complete its logic and spend its coins as intended (in our example, determine the winners and pay them their prizes). 

If the secret is published on $\Z$ in the reveal stage as intended, then the consumer's code uses $x$ to determine how the consumer's coins are distributed. And if the reveal stage fails, then the consumer uses some fallback rule to determine who gets its coins (this might be, but is not necessarily, a refund \red{is it clear that we mean that the consumer is doing the refund?}). The EVR primitive does not restrict the consumer in any way in regards to this fallback distribution. %In order for the consumer to offer good user experience / be competitive with centralized counterparts it is expected to reassure its users that in case of failure it would refund their tickets.

Accordingly, there are two opportunities for users to ``game'' the consumer and make illicit profit. First, obtaining the secret before $cnd$ matures might allow a user to ``steal'' the consumer's coins (in our lottery example, by buying the winning ticket). Second, preventing the secret from being published after $cnd$ matures opens profit opportunities from the consumer's fallback distribution. %Put differently, an entity that cannot obtain $x$ before $cnd$ matures, and that cannot prevent $x$'s publication after $cnd$ matures cannot extract \red{unfair/illegitimate} economic value from the consumer.

We restrict the potential illicit profit as formalized in the following definition. If the consumer follows these restrictions, then an EVR source \red{is guaranteed to / needs to / must} satisfy its properties. 

\begin{definition}[Single-shot EVR correct-usage]
\label{def:evrs-usage}
A correct consumer of an EVR source sets a verifiable condition, $cnd$, that matures at some point and satisfies the following conditions:
\begin{enumerate}[label=CU\arabic*.,ref=CU\arabic*]
    \item \idit{If commit fails, no user gains illicit profit.} 
    %Users who cause the failure of the commit stage cannot \red{guarantee} themselves any consumer's coins.
    \label{def:evrs-usage:commit}
    
    \item \idit{If reveal fails, the total illicit profit gained by all users is at most $P$.} 
    %Users who cause the failure of the reveal stage can \red{guarantee} themselves at most $P$ consumer's coins.
    \label{def:evrs-usage:reveal}
    
    \item \idit{If secrecy breaks, the total illicit profit gained by all users is at most $P$.}
    %A user who obtains $x$ before $cnd$ matures can \red{guarantee} herself at most $P$ consumer's coins. 
    \label{def:evrs-usage:before_cnd}
    
    \item \idit{If reveal passes and secrecy is preserved, no illicit profit is made.}
    %Assuming the reveal stage passes, a user who does not obtain $x$ before $cnd$ matures cannot \red{guarantee} herself any consumer's coins. 
    \label{def:evrs-usage:after_cnd}

    % \item For an entity (or group of entities) that does not obtain $x$ before $cnd$ matures, the only way to guarantee itself consumer's coins is by causing the failure of the reveal stage.\label{def:evrs-usage:reveal1}
\end{enumerate}
\end{definition}

\avi{ALTERNATIVE DEFINITION:}
\begin{definition}[Single-shot EVR correct-usage]
\label{def:evrs-usage}
A correct consumer of an EVR source sets a verifiable condition, $cnd$, that matures at some point and satisfies the following conditions:
\begin{enumerate}[label=CU\arabic*.,ref=CU\arabic*]
    \item \avi{If non-triviality breaks, no user gains illicit profit.}\label{def:evrs-usage:commit}
    
    \item \avi{If robustness breaks, the total illicit profit gained by all users is at most $P$.}\label{def:evrs-usage:reveal}
    
    \item \avi{If secrecy breaks, the total illicit profit gained by all users is at most $P$.}\label{def:evrs-usage:before_cnd}
    
    \item \avi{If secrecy and robustness are preserved, no user gains illicit profit.}
    \label{def:evrs-usage:after_cnd}

\end{enumerate}
\end{definition}

% There are 3 types of necessary explanations here: (i) That these restrictions are feasible to comply with. (ii) That users can check that they are indeed respected. (iii) The motivation behind these restrictions and why we have them. We mostly focus on (i) here. (ii) is trivial. We show (iii) in the analysis where we point to where these restrictions are used in the proofs. 

These restrictions are reflected in the utility functions of the game we define in \Cref{sec:game-def}. To clarify the restrictions \red{and show that they are easy to comply with}, we now illustrate them in the lottery example. 

To make sure that nothing can be gained from failure of the commit stage (\ref{def:evrs-usage:commit}), the lottery opens the ticket sale after $\E$ enters the pending stage. Note that if the ticket sale precedes the commit stage, then an attacker holding a specific set of lottery tickets that are not winners would have been able to profit from failing the \ascii{commit} protocol and getting a refund on their tickets.

By restricting the amount raised (from ticket sales) to $P$ coins, the lottery ensures that failing the reveal stage or obtaining $x$ before $cnd$ matures is worth no more than $P$ coins (\ref{def:evrs-usage:reveal} and \ref{def:evrs-usage:before_cnd}). (More generally, whenever the consumer maintains its total payouts under $P$ it satisfies the two latter conditions.)

To comply with \ref{def:evrs-usage:after_cnd}, the consumer must make sure that: (i) there is not a way to infer a winning ticket without actually having $x$, and (ii) obtaining $x$ after $cnd$ matures cannot result in illicit profits. The second item is straightforward -- by closing the ticket sale before $cnd$ matures, the lottery makes sure that obtaining $x$ after $cnd$ matures is too late to game the consumer. %(We note that the $x$ revealed implies that some lottery participants make a profit, but this is a legitimate profit that the lottery intends to distribute.)

To comply with the first item, there are two further pitfalls. First, a sophisticated user that can extract partial information about $x$ before $cnd$ matures (recall that $X$ is not a strictly hiding commitment) might permit gain an unfair advantage in the lottery. To combat this concern, an appropriate decision rule must be used (by the lottery). For example, if say $20$ of $x$'s bits can be learnt by a sophisticated player and the lottery's decision rule is $min_{tickets}\{XOR(x,ticket)\}$, then that player has a significant advantage over simple players. However, if the decision rule is $min_{tickets}\{Hash(x,ticket)\}$ then having partial information about $x$ does not help. A further study of this issue is left for future work.

Second, investors might cooperate such that together they provide $t+1$ shares (which suffices to reconstruct $x$), but within a multi-party computation (MPC)~\cite{} protocol that ensures the privacy of each investor's input (i.e., her shares) and outputs a winning ticket. The MPC ``goes through'' $x$ to compute the winning ticket, but in such a way that $x$ is never revealed to any of the investors. \red{MPCs are generally not practical to run, even in the best scenario, where there are two participating processes and they are both honest. They are theoretically possible for any function, but not necessarily practical~\cite{}. The lottery must make sure that its decision rule is not vulnerable to such an attack. Also, what does the MPC reveal about steps in the computation? If $x$ might be computed at some point, maybe it cannot be kept obscure from the participants? We need to verify this point.}

% \red{delete? We have hinted in the previous section that our solution, presented in \Cref{}, takes the form of a service in $\Z$ (i.e., a smart contract with an initial registration phase). Nonetheless, the formal description of the problem is given in general terms and is of importance for its own right. Different solutions can be devised, some of which might not require a service at all.}

% \red{delete? The EVR primitive comprises an economically-aware randomness source -- upon a consumer's request, the source emits a random value that has an \sout{explicit} economic worth. The randomness source satisfies a set of requirements (defined below) that render the value it emits secure. There are some restrictions on its usage, formalized (below) as EVR correct-usage. Thus, a solution to the EVR primitive is a randomness source that when used correctly by a consumer satisfies the EVR requirements.}

\begin{remark}
\red{Many types of cryptographic primitives can be adapted to adhere to the EVR's \red{structure/interface}. Examples include protocols that rely on classical commitment schemes (as done in \sout{this work} \idit{--put a citation or a reference to a section}), for instance, Pedersen commitments~\cite{}. Protocols that rely on computational delay or time-lock puzzles can also work -- an input to a delay function~\cite{} or a VDF~\cite{} can serve as a commitment under certain conditions, or a PoW scheme can be used. Note that in some cases, a commitment might have multiple corresponding values, each of which could be the one revealed (as in PoW).}
\end{remark}

==> trash/EVR_source_service_old.tex <==
In this section we describe our realization of the EVR primitive. 
In \Cref{sec:eth_DKG} we overview Escrow-DKG, which is a building block in our solution. Then, in \Cref{sec:EVR_realization} we present our solution. In \Cref{sec:design-rationale} we intuitively describe the design rationale that led us to make the principal choices in our solution.

\subsection{\red{Preliminaries/Background} -- Eth-DKG}
\label{sec:eth_DKG}
\sout{Secret Sharing (SS)~\cite{} is a method for distributing a secret among a group of processes. In a common $(t,n)$-SS scheme, there is a dealer and $n$ processes. Initially only the dealer holds the secret, and it sends a share to each process. Subsequently, any subset of at least $t+1$ processes that cooperate can reconstruct the secret, whereas no subset of $t$ or less processes can extract any information about the secret.} 

Distributed Key Generation (DKG)~\cite{} protocols are SS extensions that remove the dealer, and allow the processes themselves to randomly sample the secret. A DKG run produces a commitment to the secret, but the secret itself is kept obscure from all processes. Traditional $(t,n)$-DKG protocols (for example, joint-Feldman~\cite{} or Ped-DKG~\cite{}) function correctly under a model with a threshold of $t$ Byzantine processes. %Under this model, these protocols guarantee that a random secret is sampled and that an honest participant cannot be prevented from obtaining a valid share.

\red{``DKG allows a set of n servers, a.k.a. “players”, to jointly generate a pair of public and private keys in a such a way that the public key is output in the clear while the private key is shared by the n servers via a threshold secret-sharing scheme [Sha79]. Unless an adversary compromises 1 more than a specified threshold, e.g., t < n/2, out of the n servers, the generated private key remains secret and its secret-sharing can be subsequently used by these servers to jointly compute signatures or decryptions, or perform any other functionality required of the secret key in a cryptosystem. For discrete–log based threshold schemes, distributed key generation amounts to a distributed generation (i.e. without a trusted dealer) of a Shamir secret sharing [Sha79] of a random value x, and making public the value y = g x . Following [GJKR99], we refer to such a protocol as DKG.''}

Eth-DKG~\cite{rational_thresold_cryptosystems, EthDKG} is a variant of the joint-Feldman protocol, adapted to function correctly under a model of rational participants. Eth-DKG comprises a pair of protocols \ascii{generate} and \ascii{reconstruct} and an accompanying service on $\Z$, $\E$, that oversees these protocols. $\E$ establishes a set of participants during an open registration stage in which users register by depositing $1$ coin (similarly to the registration stage described in the \Cref{sec:model}). Then, the \ascii{generate} protocol runs in the background and publishes the outputted commitment on $\E$'s state (to clarify, the \ascii{generate} protocol is a DKG protocol as described above). $\E$ verifies that the commitment is correct in the sense that each registered account obtains a share that corresponds to the underlying secret. The main difference between Eth-DKG and traditional DKG protocols is that an Eth-DKG run can fail. Failure happens when $\E$ detects an inconsistency between the published commitment and the participants' shares. For $\E$ to fail, one (or more) of the participants must break the rules of the \ascii{generate} protocol. $\E$ identifies the misbehaving participant and confiscates her deposit. Correct participants get their deposits back. In doing so, $\E$ incentivizes the participants to follow the protocol's rules, and as long as they cannot obtain more than $1$ coin from failing the protocol, they are better off complying with the protocol's rules.

If failure does not happen, then a commitment, $X$, is published on $\E$'s state, and each registered account obtains a corresponding share. Then, a run of the \ascii{reconstruct} protocol can produce $x$, the secret value committed to by $X$, as long as $t+1$ shares are provided (no protocol in which $t$ shares or less are provided can reveal any information about $x$). $\E$ verifies that the published value indeed corresponds to the commitment. \red{(Note that $(X,x)$ can be a pair of public and private keys for a signature scheme. In this case, $x$ itself is not revealed, but the accounts can produce a threshold signature if $t+1$ signature shares are provided.)}

Eth-DKG has a concrete implementation in Ethereum, given in~\cite{Github_DKG_Ethereum} \cite{TheGuysFromAustria}.

\idit{Why $\E$ turned to $\G$ and the DKG to $\E$?}

\subsection{Our EVR source realization}
\label{sec:EVR_realization}

For \ascii{commit} and \ascii{reveal}, we use the \ascii{generate} and \ascii{reconstruct} protocols in Eth-DKG. We will denote these as \ascii{DKGcommit} and \ascii{DKGreveal} respectively. The smart contract that we implement, denoted $\G$, is a service in $\Z$, namely it is an escrow account with an initial registration stage in which investors register.
After registration, $\G$ adheres to the EVR source smart contract stage structure, defined in \Cref{?}. 
In Fig.~\ref{fig:G_alg} we give the pseudo-code for $\G$.
%\input{figures/EVRS_algorithm}
\input{figures/EVRS_algo_2_old}

\subsubsection{The registration stage.}
During registration, users in $\Z$ submit registration transactions that invoke $\G.\ascii{register}(acc, \$1)$. We assume that this step satisfies the definition of a service in \Cref{sec:model}.  

\subsubsection{The commit stage.}
$\G$ enters the commit stage when the consumer submits a transaction invoking $\G.\ascii{commitTrigger}(cnd)$. At this point, $\G.verCommit=false$. The \ascii{commitTrigger} function sets the necessary parameters for \ascii{DKGcommit}. Namely, $n$ is the number of shares to be generated for investors and $t=\nicefrac{2n}{3}$ is the threshold for reconstructing the secret. \ascii{DKGcommit} can now run \sout{in the background} off-chain, among the $N$ investors. The run generates $n$ shares of a secret $x$, where investor $i$ ends up with $a_i$ shares. Any $t+1$ shares (or more) can reconstruct $x$, while any $t$ shares (or less) reveal nothing about $x$. The run also generates $X$, a commitment for $x$, and publishes it on $\G$. $\G$ then verifies that $X$ is consistent with the produced shares that the investors hold (note that this verification is protocol specific; in some DKG protocols it might require more data from the \ascii{DKGcommit} run to be published on-chain, for more details see~\cite{}) and if so, updates $\G.verCommit$ to true.  

The \ascii{DKGcommit} run has $tout_1$ seconds to complete (i.e., at most $tout_1$ seconds can pass from the invocation of $\G.\ascii{commitTrigger}(cnd)$ and the update $\G.verCommit=true$). If the \ascii{DKGcommit} run fails, $\G$ enters the abort stage. Otherwise, it continues to the pending stage.  

$\G.\ascii{commitTrigger}(cnd)$ sets two more parameters: $P=n-t$ is the bound on the economic worth of the randomness, and $\ell=n$ is the framing reward, explained below.

\subsubsection{The pending stage.}
The pending stage is the crux of the protocol. The only function that can be successfully invoked in this stage is framing, $\G.\ascii{frame}(x,acc)$. Framing is key to ensuring secrecy, namely that $x$ remains secret so long as $cnd$ does not mature \sout{(as defined in \Cref{def:single-shot-EVR})}. 

Note that the incentive to break secrecy is evident -- any investor (or group of investors) that obtains $x$ before $cnd$ matures may make a substantial profit by ``stealing'' the consumer's coins (e.g., buying the lottery's winning ticket) of up to $P=n-t$ coins (by the correct-usage definition). Framing nullifies this incentive by allowing any user who knows $x$ before $cnd$ matures to publish it on $\G$'s account for a high reward of $\ell=n$ coins (line~\ref{alg:G:framing_reward}). These coins come from the investors' deposits, which are all confiscated in this case. The key property we utilize here is that in order to steal, at least one investor needs to locally reconstruct $x$. If this happens, that investor would have to make a decision -- to frame or to steal. As long as there is no investor who is better off stealing than framing, the framing mechanism is effective. It discourages investors from attempting to break secrecy as they realize that any one of them would frame if they had the possibility to do so.

We note that no side contracts can be devised that force a framer to forego or re-distribute her reward from $\G$. To clarify this subtle point, consider the following scenario, an investor that wishes to steal the jackpot might attempt to convince fellow investors to cooperate with her (i.e., send her their shares) by committing to give up the framing reward were she to frame. If possible, framing would lose its sting. Fortunately, this issue is solved by letting framers indicate an arbitrary account to transfer the reward to. Thus, a framer can always use a fresh EOA that non of the side contracts she engaged with are aware of.

If the framing function was invoked it implies that $t+1$ (or more) accounts have reconstructed $x$ while it was forbidden to do so (note that from the commitment scheme being hiding, retrieving $x$ otherwise is impossible) and can be seen as a collective punishment \red{against the investors}. The framer who ``betrays'' the collusion is rewarded for her actions. If multiple framers attempt to frame, we assume for simplicity that all of their framing transactions are submitted to $\Z$ simultaneously. $\Z$'s Log then orders the transactions according to some deterministic order and the first transaction gets executed.

If framing happens, $\G$ advances to the abort stage. Otherwise, $\G$ enters the reveal stage when $cnd$ matures.

\subsubsection{The reveal stage.}
During the reveal stage, the investors engage in a run of the \ascii{DKGreveal} protocol to reconstruct $x$. If the run completes successfully then $x$ is published on $\G$. $\G$ then verifies that the published secret is correct (i.e., that it corresponds to $X$). If this is the case, $\G$ updates $\G.verCommit=true$. The investors then get their deposits back, and $\G$ advances to the final stage. In this case, the consumer can query $\G$ for the secret value and use it. 

In case the investors fail to publish $x$ in a timely manner, $\G$ enters the abort stage. Note that in order for this to happen, investors holding at least $n-t$ shares must refrain from participating in the \ascii{DKGreveal} protocol.

\subsubsection{The final stage.}
In the final stage, the consumer, or anyone for that matter, can read $x$ from $\G$. If $\G$ enters the final stage we say that $\G$ satisfies robustness. 

\subsubsection{The abort stage}
$\G$ can enter the abort stage either because framing happens, or because the reveal stage timeouts. In both cases, all the deposits are confiscated. In case framing happens, the account indicated in the framing transaction is rewarded with $\ell=n$ coins. In case $x$ is not revealed, the coins remain in $\G$'s balance forever. Either way, if $\G$ enters the abort stage then robustness is violated.

% \begin{remark}
% \red{On a practical note, we emphasize that in both framing and the final publication of $x$, we do not require publishing individual shares on $\Z$. This allows stirring much of the computational load off-chain and enables $\G$ to reach massive scale (in terms of the number of shares generated). Also, most of the DKG's computational burden can be stirred off-chain.}
% \end{remark}

\subsection{$\G$'s Design Rationale}
\label{sec:design-rationale}
Before going into the formal analysis of $\game$ we give the intuition behind our parameters' choices: $t=2n/3$, $P=n-t$ and \red{$\ell=n$}.

First note that if $P > n-t$ then investors holding $n-t$ shares might be better off failing $\G.\ascii{DKGreveal}$ because by Property~\Cref{?}, $P$ coins can be gained from failing the \ascii{reveal} function. Since we want $P$ to be as large as possible, we define $P=n-t$.

We would also like the framing reward, $\ell$, to be as large as possible, encouraging an investor who obtains $t+1$ shares or more before $cnd$ matures to frame. We therefore set $\ell=n$, which is the total value in possession of $\G$. This might seem problematic as the framer could divide her reward among the other investors in an attempt to encourage them to cooperate with her. However, as noted in above, the inner mechanics of the framing mechanism always allow the framer to dishonor any such commitment given to other investors.

We are left with setting $t$. While a framer cannot distribute her reward, she can distribute her external coins. Additionally, in case of framing, the consumer's coins might end up in investors' hands. To make sure that framing results in losses for at least one colluding investor, it must be the case that it is not profitable to distribute $e_i + P=e_i+n-t$ coins among investors holding $t+1-a_i$ shares. The decentralization assumption takes care of this: $e_i+a_i \le 2t-n$ for all $i\in [N]$. Now, we set $t$ as to maximize both the economic worth of the randomness $P=n-t$, and the maximal investor balance allowed $e_i+a_i = 2t-n$. This leads us to set: $t=2n/3$.

\begin{remark}
Note that since we assume that a single investor can register multiple times in $\G$, assuring secrecy would be hopeless if we did not assume that for all $i\in [N]$, $a_i\le t=2n/3$. The decentralization assumption is a bit stronger: $\forall i\in [N]$, $a_i+e_i\le n/3 = t/2$.
\end{remark}

\red{Another design choice we made that might raise questions is why conduct the \ascii{DKGreveal} run off-chain and only publish $x$ on-chain. We could have had investors reveal their private shares on $\G$ and let it compute $x$. In case of success (i.e., at least $n-t$ shares are published) $\G$ would return the deposits to all investors, whereas in case of failure, the investors that did reveal their shares would get their deposits back. There are practical reasons not to do that -- gas costs and speed (in the optimistic case, the off-chain protocol can be very fast). There are also economic reasons not to do that ??..} 

==> trash/SNE_implies_CPNE_old.tex <==
Assume a game $\Gamma = \langle \{ S^j\}_{j=1}^n, \{ u^j: S \rightarrow \mathbb{R} \}_{j=1}^n \rangle$, where $S=\Pi_{j=1}^n S^j$.

For any $J \subset [n]$ and $s^0_{-J} \in \Pi_{i\in -J} S^i$ ($-J=[n] \setminus J$), define $\Gamma /\ s^0_{-J}$ to be the game induced on sub-group $J$ when sub-group $-J$ plays according to $s^0_{-J}$. Formally: $\Gamma /\ s^0_{-J}= \langle \{ S^j\}_{j \in J}, \{ u_{s^0_{-J}}^j: S^J \rightarrow \mathbb{R} \}_{j \in J} \rangle$, where: $S^J=\Pi_{j \in J} S^j$ and $u_{s^0_{-J}}^j (s_J) = u^j (s_J, s^0_{-J})$.

\begin{definition} [Strong Nash equilibrium]
$s^*\in S$ is an SNE in $\Gamma$ if $\forall J \subset \red{\subsetneq} [n]$ ($J \ne \emptyset$ and \red{$J \ne [n]$}) and $\forall s^0_J \in S^J$, $\exists i\in J$ such that $u_{s^*_{-J}}^i(s^0_J) \le u_{s^*_{-J}}^i(s^*_J)$.  
\end{definition}


\paragraph{Coalition-proof Nash equilibrium (semi-formal).}
$s^*\in S$ is a CPNE in $\Gamma$ if (1) $s^*$ is \emph{self-enforcing} in $\Gamma$ and (2) $\forall J \subset [n]$ and $\forall s^0_J \in S^J$, either (i) $s^0_J$ is not self-enforcing in $\Gamma /\ s^*_{-J}$, or (ii) $\exists i\in J$ such that $u_{s^*_{-J}}^i(s^0_J) \le u_{s^*_{-J}}^i(s^*_J)$. (2)(ii) is a straightforward check, but (1) and (2)(i) require a recursive definition -- the concept of self-enforcability relies on the concept of coalition-proofness. (The difference between a CPNE and an SNE is the fact that for every $J \subset [n]$ we only consider $s^0_J \in S^J$ that are self-enforcing in $\Gamma /\ s^*_{-J}$. We note that if $s^*$ is an SNE then it is also self-enforcing which implies that an SNE is also a CPNE.) 

Regarding (1), $s^*$ is self-enforcing in $\Gamma$ if for every $J \subset [n]$, $s^*_J$ is a CPNE in $\Gamma /\ s^*_{-J}$. But how do we know if this holds? We are in the midst of trying to define what a CPNE is. Let's use the definition we had recursively: $s^*_J$ is a CPNE in $\Gamma /\ s^*_{-J}$ if: 
\begin{itemize}
     \item case 1: $J = \{i\}$. $\forall s^0_i \in S^i$, $u_{s^*_{-J}}^i(s^0_i) \le u_{s^*_{-J}}^i(s^*_i)$.
     \item case 2: $|J| > 1$. (1') $s^*_J$ is self-enforcing in $\Gamma /\ s^*_{-J}$ and (2') $\forall J' \subset J$ and $\forall s^0_{J'} \in S^{J'}$, either (i') $s^0_{J'}$ is not self-enforcing in $\Gamma /\ s^{*,*}_{-J,-J'}$ (note that $-J' = J \setminus J'$) which is simply equivalent to $\Gamma /\ s^*_{-J'}$, or (ii') $\exists i\in J'$ such that $u_{s^{*,*}_{-J,-J'}}^i(s^0_{J'}) \le u_{s^{*,*}_{-J,-J'}}^i(s^*_{J'})$.
\end{itemize}

Regarding (2)(i), $s^0_J$ is not self-enforcing in $\Gamma /\ s^*_{-J}$ if we can find $J^1 \subset J$, such that $s^0_{J^1}$ is not a CPNE in $\Gamma /\ s^{*,0}_{-J,-J^1}$.
\begin{itemize}
    \item case 1: $J^1 = \{i\}$. It is easy to verify that $s^0_i$ is not a CPNE in $\Gamma /\ s^{*,0}_{-J,-i}$. 
    \item case 2: $|J^1| > 1$. Taking the negation from above, we would have to show that either (i'') $s^0_{J^1}$ is not self-enforcing in $\Gamma /\ s^{*,0}_{-J,-J^1}$, or (ii'') that $\exists s^1_{J^1} \in S^{J^1}$ that is self-enforcing in $\Gamma /\ s^{*,0}_{-J,-J^1}$, such that $\forall i\in J^1$, $u_{s^{*,0}_{-J,-J^1}}^i (s^1_{J^1}) > u_{s^{*,0}_{-J,-J^1}}^i (s^0_{J^1})$. 
\end{itemize}

To show (i'') we have to find $I \subset J^1$ such that $s^0_{I}$ is not a CPNE in $\Gamma /\ s^{*,0,0}_{-J,-J^1,-I}$. If we can find such $I$, we could have just taken $J^1$ to be $I$ \red{and...} %And again, if we can find $I$ of size $1$ this is easy to verify (but this shall not happen as then we could have finished in the previous step). If $I$ is of size larger then $1$ we need to continue with the inductive definition.

To show (ii'') we have need to show that a suitable $s^1_{J^1} \in S^{J^1}$ is self-enforcing in $\Gamma /\ s^{*,0}_{-J,-J^1}$. To do that, we need to show that for all $I\subset J^1$, $s^1_I$ is a CPNE in $\Gamma /\ s^{*,0,1}_{-J,-J^1,-I}$.      


% find $I \subset J^1$ such that $\overline{s^0}_{I}$ is not a CPNE in $\Gamma /\ \overline{s^{*,0}}_{-J,-J^1}$ and $\overline{s^1}_I \in S^I$ such that $\overline{s^1}_I$ is self-enforcing in $\Gamma /\ \overline{s^{*,0,1}}_{-J,-J^1,-I}$ and such that $\forall i\in I$, $u_{\overline{s^{*,0,1}}_{-J,-J^1,-I}}^i(\overline{s^1}_I) > u_{\overline{s^{*,0,1}}_{-J,-J^1,-I}}^i(\overline{s^0}_I)$.

The best way to picture this is via a tree $T=(V,E)$. The root of the tree $v_r \in V$ is a pair $(s^*, \Gamma)$. Then, at height $1$, we have vertices of the form $v_J = ((s_J^*, \Gamma /\ s_{-J}^*), S^0_J)$. The set $S^0_J \subset S^J$ includes only strategy vectors that do not satisfy condition (2)(ii), i.e., $s^0_J \in S^0_J$ if and only if $\forall i\in J$ it holds that $u_{s^*_{-J}}^i(s^0_J) > u_{s^*_{-J}}^i(s^*_J)$. All vertices $v_J$ for which $S^0_J=\emptyset$ are leaves. However, if in some vertex, $S^0_J$ is not empty we need to show that every $s^0_J \in S^0_J$ is not self-enforceable in $\Gamma /\ s_{-J}^*$. (Note that if there exists a vertex $v_J$ (of height $1$) where $J=\{ i\}$ and whose $S^0_j$ is not empty, then $s^*$ is not a CPNE. As a matter of fact, it's not even an NE.) Every vertex $v_J$ (of height $1$) where $|J| > 1$ and whose $S^0_j$ is not empty will have a predecessor, $v_{J, s^0_J}$ for every $s^0_J \in S^0_J$ from which a sub-tree whose aim is to prove that $s^0_J$ is not self-enforcing in $\Gamma /\ s_{-J}^*$ is built. To do that, we define a predecessor to $v_{J, s^0_J}$, denoted $v_{J,J^1,s^1_{J^1}} = (s_{J^1}^1, \Gamma /\ s_{-J,-J^1}^{*,0})$ which proves that $s_{J^1}^0$ is \emph{not} a CPNE in $\Gamma /\ s_{-J,-J^1}^{*,0})$. If $J^1= \{i\}$ then we verify that indeed $u_{s_{-J,-i}^{*,0}}^i(s_i^1) > u_{s_{-J,-i}^{*,0}}^i(s_i^0)$. If however, $|J^1|>1$ we verify that $\forall i\in J^1$, $u_{s^{*,0}_{-J,-J^1}}^i (s^1_{J^1}) > u_{s^{*,0}_{-J,-J^1}}^i (s^0_{J^1})$ and that $s^1_{J^1}$ is self-enforcing in $\Gamma /\ s^{*,0}_{-J,-J^1}$.


to keep extending the sub-tree. We define a predecessor to $v_{J,J^1}$   

For that we will use height $2$ of the tree: 
\begin{enumerate}
    \item We consider first vertices $v_J$ of height $1$ where $J=\{ i\}$. If $v_J.S^0_j \ne \emptyset$, then $s^*$ is not a CPNE, otherwise, we continue to height $2$.    
\end{enumerate}


\begin{definition} [Coalition-Proof Nash equilibrium]
\begin{itemize}
    \item
\end{itemize}
\end{definition}


\begin{proposition}
If $\overline{s*}$ is an SNE then it is also a CPNE.
\end{proposition}

\begin{proof}
In the case that $\overline{s*}$ is an SNE, (2) from the definition of a CPNE is always satisfied as (2)(ii) can be directly derived from the fact that $\overline{s*}$ is SNE. But this is not enough, we need to show (1), namely that $\overline{s*}$ is self-enforcing in $Gamma$. But this quite simply collapses to showing that $\overline{s*}$ is simply a NE.

In more detail we build a tree according to the order in which coalitions deviate. 
\end{proof}

==> trash/analysis_draft01.tex <==
In this section we assume that $\G$ is correctly used by some lottery $\L$, (cf.~Def.~\ref{def:evrs-usage}). Given an invocation of $\G.\ascii{init}(\beta, cnd)$ by $\L$ a game-theoretic playground is set. First, potential investors need to choose whether (and how many times) they register. We refer to this game as the \emph{registration game}. Then, if $\ascii{init}$ passes, returning $(B,X)$, each investor holds a number of shares that correspond to $x$ and they need to decide whether they send these shares to other investors while $cnd=$false in an attempt to break $x$'s secrecy. We refer to this game as the \emph{secrecy game}. Finally, if secrecy is preserved in the secrecy game, then when $\G.\ascii{getrand}()$ is called, investors engage in the \emph{robustness game}, where they need to decide whether to publish their shares or keep them obscure in an attempt to abort $\G$.

Each game is instantiated only if the previous one ends in positive terms. That is, only if the registration game ends with \ascii{init} passing (i.e., at least one investor registered) does the secrecy game begin. Then, only if the secrecy game ends such that secrecy is preserved does the robustness game begin. 

We shall define each game formally hereafter, where we depict for each game the strategies available per player, and the players' utilities given a strategy vector. In some cases, the utility of the game relies on the outcome of a following game or previous game. We depict the games in chronological order -- from registration, through secrecy, to robustness, and analyze them the other way around.

\red{Our goal is to show that each game, if played by rational players, ends in a ``positive'' way for the EVRS primitive as given in Def.~\ref{}. Particularly, in the robustness game, we show that following the protocol in a way that ensures robustness is a Strong Nash Equilibrium, and that strategic choices that jeopardize robustness are not stable. Similarly, in the secrecy game we show that given that robustness would indeed be preserved (if relevant) and an assumption on how the registration game completed, then following the protocol in a way that ensures secrecy is a Strong Nash Equilibrium, and making strategic choices that jeopardize robustness are not stable. Finally, we show that under a certain wealth distribution among potential investors, there is a Nash Equilibrium ($k$-stable strategy vector) that if followed by the investors, results in a completion of the registration game that satisfies the assumption for secrecy.}

\subsection{Background -- game theory}
\label{ssec:background}

\red{
[This part needs work (it's an outline)]
Each player has a strategy. This defines a \emph{strategy vector} 
$\overline{s} = \langle s_1, \dots, s_n \rangle$, 
where the strategy of investor $i$ is $s_i$.  
A deterministic function, known to all, determines the outcome of the game as a function of this vector. Its output includes a \emph{utility vector} $\overline{u}  = \langle u_1, \dots, u_n \rangle$, where the utility of investor $i$ is $u_i$. 
}

\red{
[This part needs work (it's an outline)]
Define: Nash, strong Nash (no coalition can deviate where no one loses and at least one profits), strategies dominating other strategies, $k$-stable. 
}


\subsection{$\G$ as a combination of three chronological games}
\paragraph{Registration game.}
The registration game follows an invocation $\G.\ascii{init}(\beta, cnd)$ by a correct lottery $\L$. We assume a universe $[N]= \{1,\dots,N \}$ of potential investors, where player $i$ has a budget of $e_i >0$ coins. The strategy set of each player is $S^1_i = \{0,1,\dots,N\}$, where we denote $i$'s choice as $a_i\in S^1_i$. $a_i$ denotes how many shares $i$ acquires, or equivalently how many times she registers within $\G$'s contract after \ascii{init} was called. $i$'s remaining budget is $e_i-a_i$ coins. Given a strategy vector $\overline{s^1}= (a_1,\dots,a_N)$, if $\sum_{i=1}^N a_i =0$, then $\forall i\in [N], u_i = e_i$ (meaning no one gains any coins) and \ascii{init} fails. Otherwise, the \idit{investors gain payoffs for partaking in $\G$. For the analysis of the current game, we assume that $i$'s payoff is proportional to $a_i$, namely, $\forall i\in [N], u_i = \alpha e_i$ for some $\alpha$. The value of $\alpha$ will be derived in ensuing sections.}
% payoffs are given by the payoffs in the strategy and robustness games, and we will give them explicitly after we analyze these games. 

\idit{By Def.~\ref{def:evrs-usage} (2)}
%From the assumption of correct usage 
it is straightforward that if $\sum_{i=1}^N a_i >0$ then \ascii{init} passes and returns some $(B,X)$. 
\idit{Which part of Def.~\ref{def:evrs-usage} does this invoke? Do you mean part 2? Then there is a strategy argument to make ... not straightforward.}
This claim holds because there is nothing to gain from failing \ascii{init}, but if $\sum_{i=1}^N a_i >0$ then failing \ascii{init} implies that whoever caused the failure loses at least $\nicefrac{1}{2}$ a coin. (As a matter of fact, this result also relies on the fact that framing never happens, as otherwise, a player that believes framing shall happen in case \ascii{init} passes is better off failing \emph{init} and losing half a coin then losing more due to framing.) From the point that \ascii{init} passes, $\G$'s global parameters are publicly available -- $n,t,B,\ell$.  

\paragraph{Analysis of the registration game given the wealth distribution assumption.}
The wealth distribution assumption: $\max_{i\in [N]} e_i < \frac{1}{4} \sum_{i=1}^N e_i$.
 
Given the analysis of the secrecy and robustness games, if $\sum_{i=1}^N a_i > \frac{3}{4} \sum_{i=1}^N e_i$ (this specifically implies that there cannot be an investor with $t+1$ shares) then the payoffs are $u_i= e_i + a_i \frac{\beta B}{n}$. Note that $B$ increases with $n$, which increases with every $a_i$ that increases. If $\sum_{i=1}^N a_i \le \frac{3}{4} \sum_{i=1}^N e_i$, then the framing mechanism might not ``work'' and secrecy could break. Then, colluding investors could steal the jackpot and the payoffs change.

We can show that playing $a_i=e_i$ is $\nicefrac{n}{4}$-stable and a Nash Equilibrium (as all investors' budget is smaller than $\frac{1}{4} \sum_{i=1}^N e_i$. This result is proven later.

\paragraph{Secrecy game.}
The secrecy game follows the registration game, and is relevant only if \ascii{init} passes. The secrecy game is played during the period where $cnd=$false. The registration game has an implicit stage zero, where registered investors can engage in agreements that define how the lottery's coins are to be distributed in case that $\G$ aborts. Recall that if $\G$ aborts, $\L$ cannot complete its logic and must fail as well, in which case at most $B$ coins can find their ways to investors' hands. Alternatively, if $\G$ does not abort, but secrecy is violated, investors may steal $\L$'s jackpot and gain up to $(1-\beta)B$ coins (on top of the coins that $\G$ distributes). 

After the agreements have been configured (in the form of a function that takes a strategy vector and returns a payoff vector $\overline{z}$ that sums up to at most $B$ or to $(1-\beta)B$), the secrecy game is defined as follows: the strategy space per registered investor $i\in [N]$ is a pair $\langle I, h \rangle$, where $I \subset [N] \setminus \{ i \}$ indicates to which investors does $i$ sends her shares, and $h$ is a function that indicates how $i$ acts given that she obtains $t+1$ shares after all investors have sent their shares. $h: I \subset (\{1,\dots, N \} \setminus \{ i \}) \rightarrow \{\overline{w}\in \mathbb{Q}_{\ge 0} \}$, where $h$ is legal if $\tickets{I\cup \{i\}}<t+1$, then $h(I)=0^N$; and if $\tickets{I\cup \{i\}} \ge t+1$ then if $h(I)=0^N$ it implies that $i$ steals the jackpot and otherwise it means $i$ frames in which case $\sum_{i=1}^N h_i(I) = ell$ is the framing reward. If indeed $i$ receives $t+1$ shares she can reconstruct $x$ locally and either frame or ``steal'' the jackpot. If she steals the jackpot the agreements from stage zero determine how the jackpot is distributed among the investors given the strategies they chose in the first entry of the secrecy game $\overline{y}(I_1,\dots,I_N) \in \mathbb{Q}_{\ge 0}$, where $\sum_{i=1}^N y_i \le B$. The theft is realized only when \ascii{getrand} is called and she publishes $x$ on $\G$'s contract. \red{(We note that the option of stealing the jackpot and then not publishing $x$ is also a viable option, but it is very unlikely and thus we overlook it.)} The payoffs are thus given as $u_i = e_i + a_i \frac{\beta B}{n} + y_i$. Conversely, if she frames, $G$ aborts which causes $\L$ to fail and the agreements from stage zero determine how $\L$'s $B$ coins are distributed among the investors given the strategies they chose in the first entry of the secrecy game $\overline{z}(I_1,\dots,I_N) \in \mathbb{Q}_{\ge 0}$, where $\sum_{i=1}^N z_i \le (1-\beta)B$. The payoffs are given by $u_i = e_i - a_i + h_i + z_i$.

she must indicate a payoff vector $\overline{w}$ that distributes the framing reward $\ell$ among the investors. (The agreements from stage zero are more limited in this regard or realistic, we do not simply let the investors do whatever they want, but limit ourselves to side contracts that are done over $\Z$. Specifically, a framer can only use its remaining balance $e_i-a_i$ in escrow accounts, etc....) In case of multiple framers, the one with the minimal enumeration is the actual framer (this is just an arbitrary choice, there can be only one framer in $\G$), and  

If secrecy is maintained, then the payoffs are determined by the robustness game. We now move to depict the robustness game and analyze it so that we can fully depict the secrecy game, analyze it and continue this way with the registration game.

\paragraph{Robustness game.}
The robustness game is played only if the two prior games ended in a specific way. The registration game ended with \ascii{init} passing, and the secrecy game with secrecy preserved. Now, the game played is very simple: there is a stage zero for agreements regarding $\L$'s coins. Then, the strategy space per investor $i\in [N]$ is $S^3_i = \{0,1\}$, where playing $0$ means that $i$ is playing counter publishing $x$ and maintains $x$ to herself, and playing $1$ means that $i$ is playing for publishing $x$ (note that there is no need to consider the case where $i$ learns the secret and only then decided whether to publish it or not as we assume there are no ``good'' results in terms of $x$ -- if $x$ is published the investors get nothing from the jackpot. Additionally, knowing $x$ early means you can steal the jackpot, so you are always incentivized to publish $x$). Given a strategy vector $\overline{s^3}$, robustness is kept if $\tickets{\overline{s^3}} \ge t+1$. The payoffs are given as follows: if $\tickets{\overline{s^3}} \ge t+1$, then $\forall i\in [N], u_i = e_i + a_i \frac{\beta B}{n}$. If however $\tickets{\overline{s^3}} < t+1$ then $\forall i\in [N], u_i = z_i(\overline{s^3})$ where $z_i$ realizes the agreements in stage zero of the robustness game.

\begin{proposition} [Robustness]
In the robustness game, the strategy vector $\forall i\in [N], s^3_i = 1$ is a strong Nash. Additionally, every strategy vector $\overline{s^3}$ such that $R(\overline{s^3}) = 0$ is not $t+1$-stable. 
\end{proposition}

\begin{proof}

\end{proof}

The previous proposition shows that investors in the secrecy game, and potential investors in the registration game, can assume that if it got to the robustness game, $x$ would indeed be published. 

Given this assumption we can complete the description of the secrecy game: If secrecy is maintained and everyone is obliged to play $h=0^N$, then the payoffs are determined by the robustness game and due to prop.~\ref{robustness}, we shall assume it results in the publication of $x$ -- $u_i = e_i + a_i \frac{\beta B}{n}$.

If the registration game ends such that $\forall i\in [N], e_i < \ell - B \sim \nicefrac{n}{4}$, we say that the registration game is \emph{healthy}.

\begin{proposition} [Framing dominant strategy]
In the secrecy game, for every investor $i$, every strategy $s^2_i$ where $s^2_i[2] = \ell \cdot \hat{e}_i$ weakly dominates every strategy $r^2_i$ such that $r^2_i[1]=s^2_i[1]$.
\end{proposition}

Prop.~\ref{} essentially says  that the framing mechanism ``works''. This means it is enough to consider strategy vectors in which $\forall i\in [N], s_i[2] =\ell \cdot \hat{e}_i$. (We set $\overline{w}$ to be $\ell \cdot \hat{e}_i$ because since side contracts cannot prevent framing we can assume they are not be used for this purpose. \red{This needs to be part of the claim as $\overline{w}$ takes into account agreements that deal with the framing reward $\ell$.})

\begin{proposition} [Secrecy]
In the secrecy game, the strategy vector $\forall i\in [N], s^2_i[1] = \emptyset$ is a strong Nash. Additionally, every strategy vector $\overline{s^2}$ such that $S(\overline{s^3}) = 0$ is not $n-t$-stable. 
\end{proposition}

\begin{proof}

\end{proof}

The previous proposition shows that if potential investors in the registration game play healthy, then secrecy is preserved. It also shows that any strategy vector that results in framing is not stable and some coalition would deviate.

We now turn to analyze the registration game. The difficulty with the registration is game is that if investors set rather small $a_i$s then the framing mechanism could be bypassed, secrecy would break, and the jackpot would be stolen. This would yield higher payoff for the colluding investors (over playing honest). The problem here is of coordination -- how does $i$ know which $a_i$ to set such that secure collusion is not risky and does $i$ know she would have a piece in the extra coins gained. All these questions are hard and are left for future work. We will show in the meanwhile that if no investor is too rich, i.e., if $\max_{i\in [N]} e_i < \frac{1}{4} \sum_{i=1}^N e_i$ then:
\begin{proposition}
In the registration game, the strategy vector $\forall i\in [N], a_i=e_i$ is $\frac{1}{4} \sum_{i=1}^N e_i$-stable and a Nash equilibrium. 
\end{proposition}

\red{\begin{remark}
We are not saying that potential investors ought to play according to this Nash, but loosely speaking, since registration is permission-less, coordination is very hard and would need to include potentially every possible coin holder in $\Z$.
\end{remark}}

We will also show that if $\sum_{i=1}^N a_i \ge \frac{3}{4} \sum_{i=1}^N e_i$, then the registration is healthy.

To show these claims one important result is that registration is \emph{risk-free}, i.e., that the chance of losing coins is $0$. This stems from the fact that was shown earlier that framing is not stable.




==> trash/analysis_old.tex <==
Intro intro ...

\subsection{Game-theoretic concepts}
\label{ssec:game-theory}

\subsection{Background}
\red{
[ToDo] 
Game, strategies, payoffs. 
A state is defined by a strategy vector $\overline{s}$. 
Extended-form game (if .. then .. clauses); $s_i$ is a vector. 
Perfect and complete [explain]

Nash, dominating strategy, Pareto domination, Coalition-proof Nash Equilibrium (CPNE), Strong Nash. 
See https://e-archivo.uc3m.es/bitstream/handle/10016/2979/we945325.pdf?sequence=1
}

\subsection{Coin stability}
\red{
Stability in terms of players is meaningless. Instead, 
a new solution concept for open settings:
\begin{definition}($k$-coin stable state)
\end{definition}
}

\subsection{The registration game}
\label{ssec:registration-game}

The registration game models the players' actions during \ascii{init}. 
It begins once a correct lottery $\L$ invokes $\G.\ascii{init}(\beta, cnd)$.
We assume a universe $U$ of players  (potential investors), where player $p$ has a budget of $e_p \in \mathbb{N}$ coins.
This is a two-stage extensive-form game. In the first stage, player $p$ 
decides on $a_p$, where $0 \le a_p \le e_p$ is the number of shares to purchase, namely, how many times $p$ registers in $\G$. Stage 1 results in some total investment being made in $\G$, denoted $n=\sum_{p \in U} a_p$. Although $n$ is derived from the strategies,  
we do not explicitly note the dependence on the strategy vector in order to make the notation less cumbersome. 

In the second stage, each player's strategy is captured by a predicate $\toF(n)$ indicating whether $p$ follows the \ascii{init} algorithm correctly, depending 
on the outcome of the first stage. 
For the analysis of the current game, we assume that in case \ascii{init} passes, $p$'s payoff is proportional to $a_p$ by some parameter $\alpha > 0$.
The value of $\alpha$ will be derived in ensuing sections. Formally,

\begin{definition} [registration RoI]
\red{The registration-RoI assumption stipulates that in case \ascii{init} passes, $\G$ returns all deposits and rewards each investor $i$ by at least $\alpha a_i$ for some $\alpha >0$.}
\end{definition}

The next proposition defines the resulting payoffs in different scenarios.
\begin{proposition} [Registration payoffs]
Assume registration-RoI.
Then, given a strategy vector, the payoff of player $p$ is given as follows:
\begin{enumerate}
    \item If $n=0$ then $u_p = e_p$.
    \item If $n>0$, $\toF_p(n)=0$, and $\toF_r(n)=1$ for some player $r \ne p$, then $u_p = e_p$.
    \item If $n>0$  and $\toF_p(n)=1$, then $u_p \le e_p -\nicefrac{1}{2}$.
    \item If $n>4\cdot \max_{r\in U} \{e_r\}$ and $\forall r\in U, \toF_r(n)=0$ then $u_p = e_p+ \alpha a_p$.
    \item If $0 < n \le 4\cdot \max_{r\in U} \{e_r\}$ and $\forall r\in U, \toF_r(n)=0$ then $u_p \ge e_p+ \alpha a_p$.
\end{enumerate}
\end{proposition}

\begin{proof}

\end{proof}

\red{For the proof we need to formally define the DKG guarantees in \cref{}, and show that they are satisfied in the appendix \cref{}. Case 3 will be explicitly stated as a property of DKG in \cref{}, and will be used here}. 

%In the first three items \ascii{init} fails, and in the last two items \ascii{init} passes. 

The \emph{default strategy} in this game is to first invest all coins in the protocol, i.e., set $a_p = e_p$ and then follow the protocol, i.e., play $\toF_p(n)=0$.
In the \emph{default strategy vector} all players play the default strategy.
The next proposition shows that this vector is stable wrt deviations of coalitions holding no more than a quarter of the coins in the game.
%$\frac{\sum_{r\in U} e_r}{4}$-coin stable.

\begin{proposition}
The strategy vector $\overline{s}$, where all players play the default strategy
%$\forall p\in U, s_p = \langle e_p, \mathbb{I}_1 \rangle$ 
is $\frac{\sum_{r\in U} e_r}{4}$-coin stable.
\end{proposition}

\begin{proof}

\end{proof}

It immediately follows that if no investor holds more than a quarter of the coins in the universe, then following the protocol is a Nash equilibrium.

\begin{corollary}
If $\max_{r\in U} \{e_r\} < \frac{\sum_{r\in U} e_r}{4}$, then the default strategy vector is a Nash equilibrium.
\end{corollary}


\subsection{The secrecy game}
\label{ssec:secrecy-game}

\subsubsection{Game definition} 

This game models the players' actions after \ascii{init} passes and while $cnd=$ false. 
The players in this game are the investors that partook in the registration,
denoted $[N] = \{ 1,\dots, N \}$. Each investor $i \in [N]$ has $a_i$ shares in the game and additional $e_i-a_i$ coins of ``outside money'' that it can use as collateral in side contracts. \red{repetitive: Note that $\sum_{i=1}^N a_i =n$, where $n$ is the total number of shares purchased during \ascii{init}.} 

Like the registration game, this game is multi-stage \red{(in extensive-form)}, where in the first stage, players sign side contracts and send shares to each other, and in the second stage they decide what to do with the shares they have obtained in the first. 
\red{
Their possible choices are wait, steal, or frame.
[ToDo: explain what is possible when]
[ToDo: in case of framing, the framer may reward other investors, as determined by a vector $\overline{w}$]
Recall that in case of multiple framers, the one with the smallest id is the actual framer.}
\idit{Make sure the protocol does this.}
%This is an arbitrary choice as there can be at most one framer according to $\G$'s rules)}





The predicates $F(\overline{s})$ and $S(\overline{s})$ indicate whether a strategy vector $\overline{s}$ results in framing or stealing, resp.

The payoffs at the end of this game are determined by (1) the outcome of the second stage, namely, whether framing took place (and in case yes, by whom), or the jackpot was stolen (again, by whom) or neither; and (2) the contracts signed and shares sent in the first stage. The payoffs have a component depending on $\G$'s payments and another depending on the environment, namely $\L$. 
The latter distributes up to $B$ coins in case of framing, since it causes the lottery to fail, up to $(1-\beta)B$ in case the jackpot is stolen, and no coins otherwise. 
The division of $\L$'s coins is modeled via two well-known functions $\overline{z}^f$ and $\overline{z}^s$, which take as parameters the identity of the framer or thieves, resp., as well as a stage 1 strategy vector $\overline{s[1]}$ (including contracts and who sends shares to whom). 
Each of these functions returns a vector indicating $\L$'s payoffs to all investors in the relevant scenario. By slight abuse of notation, where clear from the context, we omit the parameters to the functions and simply refer to the payoff of investor $i$ as ${z^f_i}$ in case $F(\overline{s})$ or ${z^s_i}$ in case $S(\overline{s})$. Note that, by \Cref{def:evrs-usage}: 
\begin{equation}
\sum_{i=1}^N z^f_i < B; \ \textrm{and} \  \sum_{i=1}^N z^s_i < (1-\beta)B.
\end{equation}

As above, we analyze the protocol assuming that it is robust and investors are rewarded based on some parameter $\alpha$, which will be derived below. Formally, 

\begin{definition}[Secrecy-RoI]
The secrecy-RoI assumption stipulates that whenever framing does not happen, $\G$ returns all deposits and rewards each investor $i$ by $\alpha a_i$ for some $\alpha >0$.
\end{definition}

The following proposition establishes the utilities in this game.
\begin{proposition} [Secrecy payoffs]
Assume secrecy-RoI. 
Then, given a strategy vector $\overline{s}$, the payoff of investor $i$ is given as follows:
\begin{enumerate}
    \item If $F(\overline{s})$ and $i$ is the framer, then $u_i = e_i - a_i + \ell - \sum_{j=1}^N w^i_j + z^f_i$.
    
    \item If $F(\overline{s})$ and $j \ne i$ is the framer, then $u_i = e_i - a_i + w^j_i + z^f_i$.
    
    \item If $S(\overline{s})$ then $u_i = e_i + \alpha a_i + z^s_i$.
    
    \item Otherwise ($\neg S(\overline{s})$ and $\neg F(\overline{s})$), $u_i = e_i + \alpha a_i$.
\end{enumerate}
\label{prop:secrecy-payoffs}
\end{proposition}

\begin{proof}

\end{proof}

\subsubsection{Game analysis} 

The \emph{default strategy} in this game is following the protocol, namely, signing no contracts, sending no shares, and framing whenever $t+1$ shares are obtained. Our goal is twofold: (1) to show that the default strategy is stable (in some well-defined sense); and (2) to rule out rogue behaviors, namely, framing and stealing the jackpot. 

First, we consider framing. We show that any strategy vector that results in framing is \red{(not $(n-t)$-coin stable)} Pareto-dominated by another strategy vector that results in no framing. In essence, this means that coalitions will avoid strategies that lead to this outcome. 

\begin{proposition}
Any strategy vector that results in framing is \red{(not $(n-t)$-coin stable)} Pareto-dominated by some other strategy vector (not necessarily stable) that results in no framing.
\label{prop:no-framing} 
\end{proposition}

\begin{proof}

\end{proof}

Second, to argue that investors do not collude to steal the jackpot, we need to rely on the framing mechanism. Intuitively, framing is a deterrent because it is a more lucrative option for the framer than stealing the jackpot, while it is much worse for the rest of the investors. In a model with no binding agreements, the only way for an investor to convince others that she will not frame is via a side contract, where she risks a large enough collateral. Such contracts are unavoidable if investors may use unbounded resources in order to break the system. To avoid such contracts, we require that the quantity of coins invested in $\G$ is sufficiently large compared to the budget each individual investor dedicates in order to manipulate the system. 
Specifically, we assume 
\begin{equation}
\forall i \in [N], e_i < \ell - B.
\label{eqn:high-participation}
\end{equation}

\red{Should this move to Putting it all together? Note that this assumption is justified by the outcome of the registration game when we assume that no player is ``too rich'' (\Cref{}).} 

We now show that assuming \Cref{eqn:high-participation}, the default strategy vector is a CPNE. We begin with the general observation that framing is always a better strategy for an individual investor than not framing.

\begin{proposition}
Assume \Cref{eqn:high-participation} holds. Then any strategy of investor $i$ where $i$ does not frame in some case when it has $t+1$ shares is dominated by a strategy that is the same except that $i$ frames in the same scenario. 
\label{prop:framing} 
\end{proposition}

\begin{proof}

\end{proof}

\red{Not sure about this: An immediate corollary from \Cref{prop:no-framing} and \Cref{prop:framing} is the following:
\begin{corollary}
Assume \Cref{eqn:high-participation} holds. Then secrecy is not breached in any  $(n-t)$-coin stable strategy vector. 
\end{corollary}}

We have seen that there is no stable scenario where rogue behavior occurs. To complement this observation, we show that conversely, following the protocol is stable.
\begin{proposition}
Assume \Cref{eqn:high-participation} holds. Then the default strategy vector is a CPNE.
\end{proposition}

\begin{proof}

\end{proof}

\subsection{The robustness game}

The robustness game analyzes the invocation of \ascii{getrand}, assuming it is called when $cnd$ = true, no investor has framed, and none had stolen the jackpot. 
%assuming the protocol does not abort beforehand, and no player knows $x$. 
The players are again the $N$ investors. 
Here, too, the strategy space includes the possibility of forming side contracts. 
In addition, each player makes a binary decision whether to partake in reconstructing the secret or not. 
The predicate $R(\overline{s})$ indicates whether in a given strategy vector 
\ascii{getrand} passes and $x$ is published on $\G$'s contract or \ascii{getrand} fails. 

%Note that discovering $x$ ahead of its publication on $\G$'s contract does not yield any advantages, since at this  

\begin{proposition}
The robustness game results in the following utilities:  
\idit{Invoke \Cref{def:evrs-usage} to argue that no player gains from knowing $x$ in case it is not published.}

\begin{enumerate}
    \item If $R(\overline{s})$ then $u_i = e_i + \frac{\beta B}{n} a_i$.
    
    \item Otherwise ($\neg R(\overline{s})$), $u_i = e_i - a_i + z_i$.
\end{enumerate}
\end{proposition}

As in the secrecy game, we again prove that violating robustness is not stable whereas the default strategy is. 

\begin{proposition}
Any strategy vector $\overline{s}$ for which $\neg R(\overline{s})$ is not $(t+1)$-coin stable.
\label{prop:no-no-robustness} 
\end{proposition}

Here, we are able to prove the stronger solution concept of Strong Nash Equilibrium. 

\begin{proposition}
The strategy vector where all players partake in constructing the secret is a Strong Nash Equilibrium. 
\end{proposition}

% Idit: removing below, we should avoid statements about what rational investors would do, and instead stick to solution concepts. 
%Together we have:
%\begin{corollary}
%Rational players will follow a strategy that ensures robustness. 
%\label{cor:robustness}
%\end{corollary}

\subsection{Putting it all together}

To analyze the complete protocol using our three games, we consider extended strategy vectors encompassing the strategies in the three phases. We start from the end of the game and work our way backward. 
From the robustness game, we get the following:

\begin{proposition}
The secrecy-RoI assumption holds in all $(t+1)$-coin stable strategy vectors. 
\end{proposition}
\begin{proof}
Consider a strategy vector (encompassing all games) where no theft or framing occurs before $cnd$ becomes true.
In this case, the robustness game is applicable, and we get that  
every $(t+1)$-coin stable strategy vector ensures robustness (by the contrapositive of  \Cref{prop:no-no-robustness}).
In case some investor does steal the jackpot, then the theft is only realized if $x$ is published, and again robustness is satisfied. 
From the protocol (line \red{add}), robustness results in a RoI of $\alpha = \frac{\beta B}{n}$ on each investor's $a_i$. 
Thus, whenever framing does not occur, $\G$ returns all deposits and also rewards each investor $i$ by $\alpha a_i$ for $\alpha = \frac{\beta B}{n}$, as needed.
\end{proof}

This justifies the modeling of payoffs in the secrecy game (\Cref{prop:secrecy-payoffs}).
\idit{We have a non-trivial step here; we need to somehow prune out all states that are not $(t+1)$-coin stable, and then consider the secrecy game in the remaining strategy space. Need to check the literature on how to do this.}
In the resulting game, no $(n-t)$-coin stable configuration results in framing (by the contrapositive of \Cref{prop:no-framing}). 

\idit{Continue to registration.}
 
 




% This result allows us to ignore the possibility of framing in analyzing registration, and thus (partially) justifies the assumption of $\alpha > 0$ in the registration game. 

==> trash/analysis_part_ii.tex <==
\subsection{More Results}
To strengthen our result, we also prove that any strategy vector $s$ that results in theft, framing or lack of robustness (i.e., if $T(s) \lor F(s) \lor \neg R(s)$) is not an SNE. 

The following lemma states that, restricted to the secrecy sub-game, a strategy vector $s$ that results in $\neg R(s)$ is not an SNE.
\begin{lemma}
Consider a strategy vector $s\in S$ for which $\neg F(s)$ and $\neg T(s)$. If $\neg R(s)$ then there exists a coalition $C$ and a deviation $(s^0_C,s_{-C})$ from which all members benefit.
\end{lemma}

\begin{proof}
If $s\in S_2$ then there is at least one investor with a negative payoff. This investor must be involved in some side contract, risking her external coins. By unilaterally relinquishing any side contracts she is involved with, she increases her payoff. We thus found a coalition that can deviate from $s$ and enjoy a net profit.

It remains to consider $s\in S_1$. Let $C$ be the set of investors who do not publish their shares in $s$. Since we assume $\neg R(s)$, $\tickets{C} \ge n-t$. 

Consider the set of investors $W$ who profit less in $s$ than had they gotten their deposits back, $W \triangleq \{ i\in[N] :\: z_i(s) + y_i(s) < a_i \}$.

We first show that $\tickets{W}\geq t+1$.
Assume by way of contradiction that $\tickets{W} < t+1$. Denote $\overline{W}=[N] \setminus W$ and note the following: 
\begin{enumerate}
    \item For all $i\in \overline{W}$, $z_i+y_i-a_i \ge 0$. This stems directly from the definition of $\overline{W}$. 
    \item $\sum_{i\in \overline{W}} z_i + y_i \leq \sum_{i\in [N]} z_i + y_i < P$. Here, the first inequality is due to the fact that $s\in S_1$. 
    \item $\tickets{\overline{W}} \geq n-t = P$, by the negation assumption. 
\end{enumerate}
Hence,
\[ 0 \le \sum_{i\in \overline{W}} z_i - a_i = \sum_{i\in \overline{W}} z_i - \tickets{\overline{W}} < P-P = 0, \]
a contradiction. We can thus conclude that $W \cap C \ne \emptyset$.


Define $J=W \cap C$ and consider a deviation of $J$ from their prescribed strategies in $s$, namely not publishing their shares, to publishing them. Under this deviation, the only investors who do not publish their shares are $C \setminus J$ and since $\tickets{W} \ge t+1$ and $W \cap (C\setminus J) = \emptyset$, we have that $\tickets{C \setminus J} < n-t$ which implies that $\ge t+1$ shares are published so robustness holds after the deviation. 

Since $J\subset W$ we know that each member in $J$ has gained a net profit from the deviation and thus $J$'s deviation shows that $s$ is not an SNE. %Additionally, the new strategy vector is self-enforcing. Any subset of investors $J_1 \subset J$ that deviates back to $s_{J_1}$ would fail robustness (as $J$ is the smallest set of investors that needs to deviate from $s$ in order to guarantee robustness) and would suffer a net loss. All in all, $J$'s deviation proves that $s$ is not CPNE in the secrecy sub-game. Remark: we cannot show that $s$ is not CPNE.
\end{proof}

\begin{remark}
We cannot strengthen the above lemma by showing that $s$ is not a CPNE in the secrecy sub-game.
\end{remark}

% \begin{lemma}
% Consider a strategy vector $s\in S$ for which $T(s)$. Then, $s$ is not self-enforcing. 
% \end{lemma}

% \begin{proof}
% We know that secrecy is violated in $s$. Consider all the investors that obtain $\ge t+1$ shares after stage 1. If at least one of them gains more from framing then her payoff in $s$, then there is an investor that can unilaterally deviate from $s$, frame and gain more.

% Otherwise, denote all the investors that gain less in $s$ then they would if they had gotten their deposits back, $W=\{ i\in [N] : u_i(s) < a_i \}$. We know that $W \ne \emptyset$. If all members in $W$ deviate from $s$ by not engaging in any side contracts and by not sending any of their shares in stage 2, secrecy would be kept in stage 1. Then, if we assume that in stage 2 an SNE is played, then, by Lemma~\ref{}, the deviating members get their deposits back and are hence better off after the deviation. 
% \end{proof}

\begin{lemma}
Consider a strategy vector $s\in S$ for which $F(s)$, and assume also that in case framing does not happen, then according to $s$, robustness holds in the second stage. Then, there exists a coalition $C$ and a deviation $(s^0_C,s_{-C})$ from which all members benefit.
\end{lemma}

\begin{proof}

\end{proof}

% \begin{theorem}
% $s\in S$ for which $\neg R(s)$, $T(s)$ or $F(s)$ is not an SNE in $\game$.
% \end{theorem}
 
% \begin{proof}

% \end{proof}

The conclusion from Lemmas~\ref{} is that investors can feel safe to register to $\G$. The main concern from the investors standpoint is that their deposits would be confiscated. This can happen only if framing happens or if robustness does not hold. When theft happens, the non-involved investors do not lose their deposits. 

==> trash/comparison_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}
% \small
\centering
\caption{\red{Comparison table of closely related work}}
\label{tab:related_work}
\begin{tabular}{@{}l|cccccc@{}}
\toprule
 & \textbf{\begin{tabular}[c]{@{}c@{}}Open\\ part\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Collusion\\ resistant\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Randomness\\ on-demand\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Round\\ complexity\end{tabular}} & \textbf{Collateral} & \textbf{\begin{tabular}[c]{@{}c@{}}Randomness\\ manipulation\end{tabular}} \\ \midrule
\begin{tabular}[c]{@{}l@{}}Randomness from\\ Bitcoin headers~\cite{bitcoin_public_randomness}\end{tabular} & miners & \begin{tabular}[c]{@{}c@{}}variance\\ selfish mining\end{tabular} & beacon & 1 block & $0$ & \begin{tabular}[c]{@{}c@{}}$O(1) \cdot$ block\\ reward\end{tabular} \\ \cmidrule(r){1-1}
\begin{tabular}[c]{@{}l@{}}Bitcoin \\ beacon~\cite{bitcoin_beacon_LIFs}\end{tabular} & miners & \begin{tabular}[c]{@{}c@{}}variance\\ selfish mining\end{tabular} & \begin{tabular}[c]{@{}c@{}}beacon\\ (1 bit)\end{tabular} & $k$ blocks & $0$ & \begin{tabular}[c]{@{}c@{}}$O(\sqrt{k}) \cdot$ \\ block reward\end{tabular}\\ \cmidrule(r){1-1}
\begin{tabular}[c]{@{}l@{}}Fair commit-\\ reveal with\\ penalties~\cite{bitcoin_fair_lottery,MPC_bitcoin}\end{tabular} & gamblers & $\checkmark$ & $\checkmark$ & \begin{tabular}[c]{@{}c@{}}$2$ rounds\\ (on-chain)\end{tabular} & $O(n^2)$ & impossible \\ \cmidrule(r){1-1}
Tournament~\cite{zero_collateral_lotteries} & gamblers & $\checkmark$ & winner & \begin{tabular}[c]{@{}c@{}}$\log n$\\ rounds\\ (on-chain)\end{tabular} & 0 & impossible \\ \cmidrule(r){1-1}
Proofs-of-delay~\cite{proof_of_delay_ethereum} & anyone? & $\checkmark$ & beacon & \begin{tabular}[c]{@{}c@{}}1 round;\\ init: ?\end{tabular} & $O(1)$ & \begin{tabular}[c]{@{}c@{}}impossible \\ (depends on init)\end{tabular} \\ \midrule
\textbf{\begin{tabular}[c]{@{}l@{}}EVR \\ (this work)\end{tabular}} & anyone & \begin{tabular}[c]{@{}c@{}}wealth distribution\\ registration\end{tabular} & $\checkmark$ & \begin{tabular}[c]{@{}c@{}}1 round;\\ init: 2 rounds\\ (optimistic)\end{tabular} & $O(1)$ & \begin{tabular}[c]{@{}c@{}}impossible\\ ($B_\L \le B$, \\ one honest)\end{tabular} \\ \bottomrule
\end{tabular}
\end{table*}

==> trash/explaining-the-game.tex <==
 When Stage 1 begins $cnd$ is false. According to the protocol, investors must not send any messages in this stage. However, a possible strategy for investor $i$ is to send her shares to another investor \red{(we make this artificial constraint, whereby an investor cannot send her shares to multiple fellow investors as we can simplify the analysis this way, while maintaining and even facilitating theft)}. An investor who obtains $t+1$ shares during Stage 1 can construct $x$ locally. She then chooses among three possible strategies: to frame, to steal the jackpot (this means that the thief has made a decision to publish $x$ when $cnd$ becomes true in order to realize her theft), or to simply wait for the next stage. Investors who do not obtain $t+1$ shares during Stage 1, must wait.
    
Stage 2 handles revealing the secret when $cnd$ becomes true and \ascii{getrand} is invoked. The strategies here are either to cooperate to reconstruct (and publish) the secret, or not. This stage is relevant only so long as neither framing nor stealing has occurred in stage 1. In case framing occurred, $\G$ aborts, and so the stage is trivial (i.e., has no impact on the game's outcome). And theft implies that the thief publishes $x$, so again the stage is trivial. 


\red{Note that in this description of the game, this stage is played simultaneously by all investors, while in practice certain investors could wait and reconstruct $x$ locally prior to making a decision to cooperate. To overcome this hurdle we assume the existence of an oracle that reveals $x$ to all investors before they make their decision in this stage.} 



The investors' payoffs depend on a few things: (i) Our EVRS solution, that only cares about these outcomes (and not on the exact strategies that investors choose). (ii) Side contracts formed by the investors. Coins that investors kept aside may be used in side contracts and allocated as they specify. (iii) Lottery coins. In case the EVRS aborts, the lottery is forced to abort as well, and the $B$ coins that it was supposed to allocate have an unclear destination, and might end up in investors hands. 


We now define $\game$'s payoffs. $u_i: \Pi_{i=1}^N S_i \rightarrow \mathbb{Q}$, the payoff function for investor $i$, is given as follows: 
\begin{itemize}
    \item If $F(s)$ and $i$ is the framer, then $u_i = \ell - \sum_{j=1}^N w^i_j + z^{ab}_i$. $\ell$ is the framing reward paid by our EVRS contract on expense of the investors' deposits. The framer though may compensate others via her outside coins, $e_i$. This is manifested by $\overline{w^i}$. And $\sum_{i=1}^N z^{ab}_i \le B$, where ``ab'' stands for abort.  
    
    \red{Note that the $\ell$ coins obtained from framing are not split among the investors, because the framer cannot bind herself to splitting her reward -- this is part of how our EVRS contract is designed.}
    
    \item If $F(s)$ and $j \ne i$ is the framer, then $u_i = w^j_i + z^{ab}_i$.
    
    \item If $S(s)$ then $u_i = (1+\alpha)a_i + z^s_i$. $(1-\beta)B$ is the total amount stolen, which, in whole or in part, is divided among the investors. Thus, $\sum_{i=1}^N z^s_i = (1-\beta)B$, where ``s'' stands for theft. Theft implies that $x$ is published and thus $\beta B$ is paid to the EVRS contract which allocates it to the investors, thus $\alpha = \frac{\beta B}{n}$. 
    
    \item If $\neg S(s)$, $\neg F(s)$, and $R(s)$, then $u_i = (1+\alpha)a_i$. This is the desired result from the standpoint of the designers of the system.
    
    \item Otherwise, $\neg S(s)$, $\neg F(s)$, and $\neg R(s)$. And $u_i = z^{ab}_i$.
\end{itemize}

It is important to emphasize that while each investor might not be aware of her own utility, or of her fellow investors utilities (as side contracts might be obscure from certain investors), we assume that investors cannot be ``fooled'', namely, they cannot be tricked into thinking that if some strategy vector is played they would gain a specific sum and then get paid another sum if that strategy vector was indeed played.


We assume the game to be of incomplete information. A player knows her own utility function given all the initial conditions, and they know the bounds regarding $z^{ab}$, $z^s$, etc.

We argue that the game $\game$ correctly captures our solution \red{in a pessimistic view of the investors.}  
\begin{lemma}
$\game$ correctly models the possible payoffs arising following a successful \ascii{init} invocation in \Cref{alg:evrs}, when used correctly as defined in \Cref{def:correct-usage}. 
\end{lemma}









\begin{proposition} 
There exists no self-enforcing strategy vector that is better than $s^*$ for all investors.
\label{prop:default-is-best}
\end{proposition}


\begin{proof}
We need to show that 
(1) $s^*$ is self-enforcing and (2) there is no other self-enforcing 
strategy vector that Pareto dominates $s^*$. 
We prove (2) in \Cref{prop:default-is-best}. 

We now prove (1). 
We need to show that $\forall J \subset [N]$, $\overline{s}^*_J$ is a CPNE in
$\G' /\overline{s}^*_{-J}$. We prove this by induction on $|J|$. 
Base: If $|J| = 1$, the condition for a single-player game holds because the payoffs do not change and a single investor does not hold too many shares \red{formalize}.

Step: (a) holds by induction. To prove (b) we show that there is no deviation to another self-enforcing strategy vector that is advantageous to all members of $J$. We divide the possible deviations into three cases: (i) waiting is not better for anyone as payoffs do not change; (ii) stealing is not self-enforcing by \Cref{prop:framing-works}; and (iii) framing results in lower payoff for at least one investor in $J$. \red{prove}. 
\end{proof}

\begin{proof}
Assume by contradiction that there is a self-enforcing strategy vector $\overline{s'}$ 
s.t. $\forall i \ [N], u_i(\overline{s'}) > u_i(\overline{s}^*)$. 
We consider three cases: 
\begin{itemize} 
\item $F(\overline{s'})$: We show that $\overline{s'}$ is not better for some player \red{complete}
\item $S(\overline{s'})$: by \Cref{prop:framing-works}, $\overline{s'}$ is not self-enforcing 
\item The remaining case is that neither framing nor stealing occur. In this case, 
no player has a higher payoff than in $\overline{s}^*$. 
\end{itemize}
\end{proof}

%Consider three cases: 
%\begin{itemize}
%    \item If $J$ holds less than $t+1$ shares 
%    $\neg S(\overline{s}^*_J) \wedge \neg F(\overline{s}^*_J)$ in 
% $\G' /\overline{s}^*_{-J}$, 
%    then (a) holds by induction because every subset of $J$ holds less than $t+1$ shares,  
%    and (b) holds because the payoffs cannot change by deviation     \red{justify}.
%    \item If $J$ holds at least $t+1$ shares and every proper subset of $J$ holds at most $t$ shares. Then, (a) holds by induction. To prove (b) we show that there is no deviation to another self-enforcing strategy vector that is advantageous to all members of $J$. We divide the possible deviations into three cases: (i) waiting is not better for anyone as payoffs do not change; (ii) stealing is not self-enforcing by \Cref{prop:framing-works}; and (iii) framing results in lower payoff for at least one investor in $J$. \red{prove}. 
%    \item If $J$ holds more than $t+1$ shares and has a subset with more than $t+1$ shares, (a) follows from the previous case by induction. 
    %To show that  $\overline{s}^*_J$ is a CPNE in $\G' /\overline{s}^*_{-J}$
%\end{itemize}

\begin{proposition} 
\red{Any strategy vector that results in stealing is not self-enforcing.}
%Any strategy vector $\overline{s}$ s.t.\ $F(\overline{s})$ is not self-enforcing.
\label{prop:framing-works}
\end{proposition}
\begin{proof}
\red{The idea is simple. If theft happens, than at least one investor knows $x$ before $cnd$ is true. That investor can frame, and is better off framing.}
\end{proof}

% \begin{proposition} [$\overline{s^*}$ is self-enforcing]
%For any subset of investors $J\subset [N]$, $\overline{s_J^*}$ is self-enforcing in the game $\G \/ s_{-J}^*$. 
%\end{proposition}
% \begin{proposition} [$\overline{s^*}$ dominates every other CPNE]
%There is no other self-enforcing strategy vector $\overline{s}$.
%\end{proposition}

==> trash/game_justifications_lat_actor.tex <==
\paragraph{Side contracts.}
In $\game$, investors can use any coins they still posses after the \ascii{commit} (namely their ``outside'' coins, $e_i$ for investor $i$) in order to encourage fellow investors to act in certain preferable ways. Specifically, these coins can be used in \emph{side contracts} to eliminate any trust issues among the investors. $\game$'s payoffs rely on side contracts that investors have chosen to use, and we assume no new contracts can be formed or used after the fact.

There are a few explicit assumptions regarding the smart contracts that investors can arrange:
\begin{enumerate}
    \item \sout{$\forall i\in [N]$ and $\forall s\in S$ :\: $u_i(s) \ge 0$. Explanation: We make a distinction here between investors' ``inside'' and ``outside'' coins. Investor $i$ regards her outside coins, $e_i$, as an amount she is not willing to lose. On the contrary, the $a_i$ deposit is seen as owned by the contract and as a potential profit for the investor. Since investors can always avoid risking their outside coins, we assume this is what they do indeed. More precisely, this means that an investor would never engage in a smart contract for which there is some strategy vector in which they end up with a negative payoff. Alternatively: we consider ``realisric'' strategy vectors as ones where none of the investors end up with a negative payoff.} Instead: $\forall i\in [N]$ and $\forall s_{-i}\in S$ $\exists s_i \in S_i$ :\: $u_i(s_i,s_{-i}) \ge 0$. This means that no investor can be forced to end up with a net loss. 
    
    \item $\forall i\in [N]$ and $\forall s\in S$ :\: $z_i(s)$ do not depend on the secret $x$.
    
    \item No re-distribution of EVRS coins (namely of the $a_i$s), whether they are  returned to a single framer or to all investors. Specifically, when framing happens, the framing reward ($\ell$ coins) goes solely to the framer which does not divide them among the investors. The reason for this restriction is that by the nature of the contract, the framer cannot bind herself to a strategy where she indeed splits the framing reward among the investors. This stems from the feature of the contract where any account (including non registered ones) can frame. 
    
    Similarly, when our EVRS contract returns $a_i$ coins to investor $i$, they do not further divide them. The reason is that a mechanism whereby the investors cannot be prevented from withdrawing their deposits to private accounts can be devised. (For instance, each registration transaction would include an account, where only by providing the signature for that account one could pull the deposited coins. \sout{Note that we do not consider cases in which players simply register with an account that they cannot generate a signature for.}) 
    \item \red{The side contracts are deterministic.}
\end{enumerate}

\paragraph{Strategies.}
We have restricted and simplified investors' strategies as specified hereafter.
\begin{enumerate}
    \item Stage 1. An investor that chooses to send her shares must send all of her shares to a single other investor. Note that this seemingly artificial restriction to investors' strategy sets maintains secrecy violations by any set of $\ge t+1$ shares, and by any investor. It only eliminates cases where multiple investors break secrecy simultaneously and now pose a risk to one another. This restriction facilitates breaking secrecy during stage 1.
    
    \red{Q: Is this discussion necessary if we prove a CPNE? Also, since we assume that this stage is played simultaneously by all investors, no investor can act as a ``last actor'', basing her decision in this stage on how her fellow investors have chosen to play. We could have defined an equivalent game where the investors must play according to some predefined order. Actually, our analysis would hold for any predefined order. The idea is that if we defined a sequential game where investors decide to whom to send their shares in turns, then the first investor that cannot guarantee a net profit from having some other investor frame, would keep her shares private (because the following investors would definitely take advantage of the opportunity given to them). It is a zero-sum game at the end of the day. The question here is: Do investors have an incentive to wait to play last? The answer is: No, no matter which order is considered, every investor would act the same way.)}   
    
    \item Stage 2. An investor can either publish all of her shares or none of them. This makes sense because at the end of the day, $x$ is either published or it is not. Thus, an investor that prefers $x$ to be published has no reason to keep some of her shares obscure, and vice versa, they have no reason to publish any of their shares if they prefer robustness to fail.
    
    \red{Q: Is this discussion necessary if we prove a CPNE? Also, since we assume that this stage is played simultaneously by all investors, no investor can act as a ``last actor''. Here, there are two aspects to consider. The first is similar to the previous case, but here there is also the issue with reconstructing $x$ first and making a decision to publish/withdraw according to the value found. We claim however, that this extra information is irrelevant to the decision. Both, $z_i$ and $a_i$ do not depend on the value of $x$. As a matter of fact, in case $x$ is published the payoff might be higher for the last actor (as they might find out they win the lottery) so setting the payoff to be $a_i$ is a worst-case assumption. It is as if all investors are ``last actors'' that have found a non-preferable $x$ and are thus pushed towards failing robustness.
    Put differently: Let $s_1,s_2\in S$ such that $\neg T(s_1)$, $\neg T(s_2)$, $R(s_1)$ and $R(s_2)$, then $\forall i\in [N] :\: u_i(s_1)=u_i(s_2)$.}
\end{enumerate}

\paragraph{Payoffs.}
\sout{We identify three sources of coins -- deposits in our EVRS contract, the lottery's coins $B$ and investors ``outside'' coins.}   
\begin{enumerate}
    \item \sout{EVRS coins are straightforward to analyze as the contract specifies exactly what happens with them. They cannot be re-distributed as explained in the side contracts restrictions subsection above.}
    
    \item \sout{The upper bound on the sum of the $z_i$s is due to the lottery's coins, which are the only external source of coins. In case of secrecy and robustness we assume non of these coins end up in investors' hands (which is a worst-case assumption regarding investors payoffs in this case), while in all other cases we do not assume anything on where these coins end up.}
    
    \item \red{\sout{Regarding the investors' knowledge of the game and its payoffs, we assume that the investors are not aware of their fellow investors' utility functions (i.e., the investors are only aware of the side contracts that they are a part of). This is referred to in the literature as an incomplete game. Where do we use this assumption?}}
    
    \item \red{\sout{Investors are pessimistic. Where do we use this assumption?}}
\end{enumerate}




\begin{remark} \red{Repetitive.} \sout{(Last actors are not interesting in the secrecy sub-game)
We could have illustrated $\game$ as a sequential game in which the investors are organized in some predetermined order and play their move according to that order. The information sets in this game would be singletons (i.e., perfect information game, where every investor knows the moves made by all previous investors). In such a game and regardless of the order chosen, a coalition holding $\ge n-t$ shares that refuses to publish their shares would never form. Moreover, an investor would always play the same way, regardless of the order chosen. This can be proven with backward induction.}
\end{remark}

==> trash/game_theoretic_concepts.tex <==
In this section we define the game theoretic concepts we use in our analysis.
First, a $n$-player game $\Gamma$ is a pair $[ \{ S^i \}_{i=1}^n, \{ u^i: \prod_{i=1}^n \rightarrow \mathbb{R}\}]$. $S^i$ is the strategy set for player $i$ and $u^i$ is $i$'s payoff function, which takes as input a strategy vector $s$ (namely, a vector of $n$ entries that indicates each player's decisions), and outputs $i$'s payoff. 

It is common for games to proceed in \emph{stages}, where in a stage some or all players make decisions and some new information is presented to some or all of the players before the game advances to the following stage. A multi-stage game must explicitly indicate what is known to which player at every stage. A common distinction is between perfect and imperfect information. In a multi-stage game, a player's strategy is commonly described as a set of conditions that specify which move the player chooses per stage given the evolution of the game thus far.

When analysing multi-stage games, the notion of \emph{proper subgames} is key.  

The following definitions relate to the game $\Gamm$.
\begin{defintion} [Nash Equilibrium]
$s^*$ is a NE if for every $i \in [n]$ and for every $s_i \in S^i$, $u^i(s^*) \ge u^i(s_i,s_{-i}^*)$.
\end{defintion}

In multi-stage games, the NE behavior of individual players may be \red{dynamically inconsistent}. A better concept is that of a SPE. 
\begin{defintion} [Subgame Perfect Equilibrium]
$s^*$ is a SPE if it represents a NE when restricted to any proper subgame.
\end{defintion}

NE strategy vectors do not take into account deviations of coalitions. In many games, by devising self-enforcing agreements, coalitions can deviate from their NE strategies while increasing the individual payoff of every coalition member. In such cases a NE is not a very strong solution to a game.

For such cases, stronger equilibria were devised.
\begin{defintion} [Strong Nash Equilibrium]
$s^*$ is a SNE if for every $J \subseteq [n]$ and for every $s_J \in \Pi_{j\in J} S^j$, there exists $i\in J$ such that $u^i(s^*) \ge u^i(s_J,s_{-J}^*)$.
\end{defintion}

In words, in any coalition $J$ that considers deviating from $s^*$, and for any considered new strategy by that coalition $s_J$, there is at least one member $i\in J$ that is not better off by the deviation. 

The SNE rarely exists because there is no explicit requirement that $s_J$ be self-enforcing. It might be the case that indeed all the members in the coalition profit from the deviation, but that the deviation introduces the opportunity for yet another coalition to deviate once again and ensure even larger payoffs. The following concept tackles this problem.

\begin{defintion} [Coalition-Proof Nash Equilibrium]

\end{defintion}

As with NE strategy vectors, also CPNE strategy vectors do not consistently conform to mutli-stage games. In multi-stage games we consider Perfectly CPNE strategy vectors, or strategy vectors that are CPNE in every subgame.  


==> trash/multi-shot_EVRS.tex <==
The motivation to define a multi-shot EVR source, in which a single commitment corresponds to multiple values in sequence is not clear. Why not just use a single-shot EVR source multiple times. The answer has two parts: (i) the \ascii{commit} protocol can be much more expensive and less efficient to run; and (ii) the \ascii{commit} protocol is much cheaper to fail and so it would be hard for a consumer to comply with item \ref{def:evrs-usage:commit} in the correct-usage definition. We give an example to elaborate on the second point. Imagine a $n$-player two-round die game. Before the game starts players buy tickets, then in the first round they each toss a die and make an additional bet given what they got. In the second round they each toss again and the winner that sweeps all of the money raised is the one whose sum of tosses is the largest. A player that got a $1$ in the first toss has a strong incentive to fail and get a refund. If the cost of failing the \ascii{commit} run in the second round is low it might be worthwhile. In a multi-shot EVR source, the randomness for all future rounds is set in a way that preventing the publication of any round's randomness is expensive.   

\subsection{Background -- Verifiable Random Functions}
\label{VRF_background}

Generally speaking, a VRF~\cite{VRF} is a pseudorandom function supplemented with a publicly verifiable proof. Unlike pseudorandom functions, VRFs do not permit their evaluators to ``lie'' regarding the output (by manipulating the input) and can be used to generate unbiased random values.   
We give a simplified definition of a VRF: 

\begin{definition} [VRF]
A VRF is a triplet of efficient algorithms:
\begin{itemize}
    \item $(PK,SK) \xleftarrow{R} \ascii{Gen}$,
    \item $\sigma \leftarrow \ascii{Eval}(SK,m)$,
    \item and a boolean function $\ascii{Ver}(PK,m,\sigma)$
\end{itemize}
Consider $(PK,SK) \xleftarrow{R} \ascii{Gen}$, then the three algorithms satisfy the following properties:
\begin{enumerate}
    %\item Domain-Range Correctness. If $x_1$ and $x_2$ are of the same lengths then so are $F(SK,x_1)$ and $F(SK,x_2)$. 
    \item Complete Provability. For all $m$, if \ascii{Eval}$(SK,m)=\sigma$ then \ascii{Ver}$(PK,m,\sigma)=\emph{true}$.
    \item Unique Provability. For every $m,\sigma_1,\sigma_2$, such that $\sigma_1 \ne \sigma_2$, either \ascii{Ver}$(PK,m,\sigma_1)=\emph{false}$ or \ascii{Ver}$(PK,m,\sigma_2)=\emph{false}$.\footnote{In the original definition \ascii{Ver} is a probabilistic algorithm and properties (1) and (2) hold with overwhelming probability in the security parameter. \avi{This is true to all of the properties}}
    \item Residual Pseudorandomness. There does not exist an efficient algorithm that receives $PK$ as input and after selecting some $m$ (as it pleases), can distinguish between $\sigma=\ascii{Eval}(SK,m) \in \{0,1\}^h$ and a bit-string sampled uniformly at random from $\{0,1\}^h$. 
\end{enumerate}
\end{definition}

It can be shown that a unique signature scheme realizes a VRF (see~\cite{VRF}). We will use a specific BLS-3 signature scheme as a VRF in our prototype implementation (see ~\ref{}). 


\subsection{Multi-Shot EVRS Interface and Guarantees}
Multi-shot EVRS executes a commit phase, similarly to a single-shot EVRS, but with (possibly) multiple reveal phases. 

Consider a VRF $(\ascii{Gen},\ascii{Eval},\ascii{Ver})$ and let $cnd^l = (cnd_1,\dots,cnd_l)$ be a list of $l$ verifiable conditions in $\Z$, and $(m_1,\dots,m_l)$ be a list of $l$ \sout{publicly available} predetermined bit strings.

A multi-shot EVRS exposes the following interface:
\begin{enumerate}
    \item A call $\ascii{commit}(cnd^l)$ either fails or passes within a predetermined time limit. In case it fails it returns `fail'. In case it passes it returns a pair $(P, PK)$, where $PK$ is a public key generated along with a secret key $SK$ in the execution of $\ascii{Gen}$, and $P\in \mathbb{N}_0$ indicates an economic value (in $\Z$ coins).
    
    \item A call $\ascii{reveal}(i)$, for $1 \le i \le l$, either fails or passes within a predetermined time limit. In case it fails it returns `fail'. In case it passes it returns the value $\sigma_i$, such that $\ascii{Ver}(PK,m_i,\sigma_i)=True$ (namely, it returns $\ascii{Eval}(SK,m_i)$).
    
\end{enumerate}


    

\begin{definition}[Multi-shot EVR Source]
An escrow account $\E$ in $\Z$ is a multi-shot EVRS if it implements the multi-shot EVRS interface such that the following properties hold:
\begin{enumerate}

    \item Non-triviality. A call $\E.\ascii{commit}(cnd^l)$ \red{(before $cnd$ matures)} passes. 
    
    \item (multi-shot) Secrecy. For all $1 \leq i \leq l$, if $\E.\ascii{commit}(cnd^l)$ passes, then before $cnd_i$ matures no \red{user} obtains any information about $\sigma_i$. 
    
    \item (multi-shot) Robustness. For all $1 \leq i \leq l$, if $\E.\ascii{commit}(cnd^l)$ passes, then after $cnd_i$ matures, a call $\E.\ascii{reveal}(i)$ passes and returns $\sigma_i$.
\end{enumerate}
\end{definition}

% A consumer has a few restrictions it must respect in order for the EVRS to satisfy its properties, as we now define:
% \begin{definition}[Correct usage of a single-shot EVRS]
% \label{def:evrs-usage}
% A correct consumer of an EVRS sets $cnd$ such that:
% \begin{enumerate}[label=C\arabic*.,ref=C\arabic*]
%     \item No coins can be gained from the failure of \ascii{commit}. \label{def:evrs-usage:commit}
%     \item No coins can be gained from obtaining $x$ after $cnd$ matures. \label{def:evrs-usage:after_cnd}
% \end{enumerate}

% In addition, it restricts the value of the randomness as follows:
% \begin{enumerate}[label=B\arabic*.,ref=B\arabic*]
%     \item Less than $B$ coins can be gained from the failure of \ascii{reveal}. \label{def:evrs-usage:reveal}
%     \item Less than $B$ coins can be gained from obtaining $x$ before $cnd$ matures. \label{def:evrs-usage:before_cnd}
% \end{enumerate}
% \end{definition}

\begin{definition}[Correct usage of a multi-shot EVR Source]
A correct consumer of an EVRS sets $cnd^l$ such that:
\begin{enumerate}[label=C\arabic*.,ref=C\arabic*]

    \item No coins can be gained from the failure of \ascii{commit}. 
    \item For all $1 \leq i \leq l$, no coins can be gained from obtaining $\sigma_i$ after $cnd_i$ matures. 
    
\end{enumerate}

In addition, it restricts the value of the randomness as follows:
\begin{enumerate}[label=B\arabic*.,ref=B\arabic*]

    \item For all $1 \leq i \leq l$, less than $P$ coins can be gained from the failure of $\ascii{reveal}(i)$. 
    \item For all $1 \leq i \leq l$, less than $P$ coins can be gained from obtaining $\sigma_i$ before $cnd_i$ matures.
    
\end{enumerate}
\end{definition}



\avi{
Remark: 
Note that we restrict $l < \infty$, even though in some cases (e.g., blockchains) random values are perpetually generated. Fundamentally, no entity can participate for unlimited time nor afford an endless execution of the EVRS until getting paid. Therefore, in these cases randomness generation should be split into segments, where in each segment a fresh EVRS is initiated and $l \in \mathbb{N}$ random values are produced. If the set of EVRS' participants is fixed, then redoing the \ascii{commit} procedure is unnecessary. Surly, further optimizations can be made when executing several multi-shot EVRSs in sequence, but we leave it for future work.
}

==> trash/multi-shot_EVRS_new.tex <==

Up to this point, for simplicity, we focused on a randomness source that produces a single random value. In principle, such a source may be used also by applications that require a sequence of random values, such as card and die games. However, this approach is undesirable for two reasons. First, \ascii{commit} is the most expensive part of the protocol, and in fact, it is the only protocol stage when disputes might need to be handled (as part of the DKG). We would like to limit this cost  to once per dAPP instead of once per random value generated. Second, our incentive structure  explicitly leverages the fact that no illicit profits can be made by failing \ascii{commit} (\ref{def:evrs-usage:commit}). It is easy to establish this when \ascii{commit} is executed once in a dApp, before the game begins. But as a game unfolds, a player might discover, for instance, that she is likely to lose, creating an incentive for failing the protocol. We therefore construct a \emph{multi-shot randomness source}, which may reveal a sequence of random values following a single \ascii{commit}.

% The motivation to define a multi-shot EVR source, in which a single commitment corresponds to multiple values in sequence is not clear. Why not just use a single-shot EVR source multiple times. The answer has two parts: (i) a \ascii{commit} run can be expensive and slow; and (ii) a \ascii{commit} run is cheap ($O(1)$ coins) to fail and so it would be hard for a consumer to comply with item \ref{def:evrs-usage:commit} in the correct-usage definition. We give an example to elaborate on the second point. Imagine the following $n$-player two-round die game: Before the game starts players buy their seats by contributing $1$ coin to a common pool, then in each round, each player tosses a die, where the player with the highest sum sweeps all the coins raised. The game needs two random values, one per each round (where each player uses a combination of some private input and the random value in order to find out the outcome of her toss). A player that reserved four seats in the game and got all $1$s in the first toss has a strong incentive to fail the second round and get a refund. If that player is also an investor in the EVR source and the cost of failing the \ascii{commit} run in the second round is low it might be worthwhile. In a multi-shot EVR source, once the first \ascii{commit} run passes, it is expensive to fail any subsequent \ascii{reveal} run and so it is expensive to prevent the application from reaching its intended ending. 

\subsection{Background -- Verifiable Random Functions}
\label{VRF_background}
Generally speaking, a VRF~\cite{VRF} is a pseudorandom function supplemented with a publicly verifiable proof. Unlike pseudorandom functions, VRFs do not permit their evaluators to ``lie'' regarding the output (by manipulating the input) and can be used to generate unbiased random values.   
We give a simplified definition of a VRF: 

\begin{definition} [VRF]
A VRF is a triplet of efficient algorithms:
\begin{itemize}
    \item $(PK,SK) \xleftarrow{R} \ascii{gen}$,
    \item $\sigma \leftarrow \ascii{eval}(SK,m)$,
    \item and a Boolean function $\ascii{ver-VRF}(PK,m,\sigma)$
\end{itemize}
Consider $(PK,SK) \xleftarrow{R} \ascii{gen}$, then the following properties hold:
\begin{description}
    

    %\item Domain-Range Correctness. If $x_1$ and $x_2$ are of the same lengths then so are $F(SK,x_1)$ and $F(SK,x_2)$. 
    \item[Complete Provability] For all $m$, if \ascii{eval}$(SK,m)=\sigma$, then $\ascii{ver-VRF}(PK,m,\sigma)=\emph{true}$.
    \item[Unique Provability] For every $m,\sigma_1,\sigma_2$, such that $\sigma_1 \ne \sigma_2$, either \ascii{ver-VRF}$(PK,m,\sigma_1)=\emph{false}$ or \ascii{ver-VRF}$(PK,m,\sigma_2)=\emph{false}$.\footnote{In the original definition \ascii{ver-VRF} is a probabilistic algorithm and properties (1) and (2) hold with overwhelming probability in the security parameter.}
    \item[Residual Pseudorandomness] There does not exist an efficient algorithm that receives $PK$ as input and after selecting some $m$ (as it pleases), can distinguish (with non-negligible advantage) between $\sigma=\ascii{eval}(SK,m) \in \{0,1\}^h$ and a bit-string sampled uniformly at random from $\{0,1\}^h$.
\end{description}
\end{definition}

It can be shown that a unique signature scheme realizes a VRF (see~\cite{VRF}). We will use a specific BLS signature scheme as a VRF in our prototype implementation (see \Cref{sec:implementation}). 


\subsection{Multi-Shot EVR Source and Correct-Usage}
Similarly to a single-shot EVR source, a multi-shot EVR source, has a single commit stage, but then it has (possibly) multiple consecutive reveal and pending stages.

% Consider a VRF $(\ascii{Gen},\ascii{Eval},\ascii{Ver-VRF})$ and let $cnd^l = (cnd_1,\dots,cnd_l)$ be a list of $l$ verifiable conditions in $\Z$, and $(m_1,\dots,m_l)$ be a list of $l$  predetermined bit strings.

\begin{definition}[Multi-shot EVR source]\label{def:multi-shot-EVR}
A multi-shot EVR source consists of \ascii{commit} and \ascii{reveal} protocols and a smart contract $\E$ in $\Z$.
$\E$'s variables include $l+1$ (constant) timeout periods (in seconds), $tout_{com}$ and $(tout_{rev}^1,\dots,tout_{rev}^l)$; $l+1$ Boolean variables $verCommit$ and $(verReveal_1,\dots,verReveal_l)$. $\E$'s functions include $\ascii{commitTrigger}(cnd^l, m^l)$,where $cnd^l = (cnd_1,\dots,cnd_l)$ is a list of $l$ verifiable conditions in $\Z$, and $m^l = (m_1,\dots,m_l)$ is a list of $l$ bit strings.\footnote{For simplicity, we designate the strings $m^l$ as input for $\E$. However, these strings can be hard-coded into $\E$ or dynamically generated. The only constraint in this respect is that every $m_i$ is published prior to $cnd_i$ maturing.}
$\E$ advances in the following stages: 
    \begin{description}
        \item[Commit] A call $\E.\ascii{commitTrigger}(cnd^l, m^l)$ initiates the commit stage. The commit stage lasts at most $tout_{com}$ seconds, during which a \ascii{commit} run takes place \sout{(the run may invoke on- and off-chain computations)}. The commit stage ends successfully when $verCommit$ turns \emph{true} (which implies that a valid commitment produced by the \ascii{commit} run, $PK$, is published on $\E$). However, if $tout_{com}$ seconds pass before this happens, then the stage fails. In the successful case, $\E$ designates a value $P\in \mathbb{N}$, which indicates the economic worth of the randomness (in $\Z$'s coins), and enters the first pending stage. In case of failure, $\E$ enters the abort stage.
        
        \item[Pending_i] The $i$th pending stage lasts until $cnd_i$ matures, and then $\E$ enters the $i$th reveal stage.
        
        \item[Reveal_i] The $i$th reveal stage ends at most $tout_{rev}^i$ seconds after $cnd_i$ matures. During this time, a \ascii{reveal} run takes place \sout{(the run may invoke on- and off-chain computations)}. The reveal stage ends successfully when $verReveal_i$ turns \emph{true} (which implies that the value produced by the $i$th \ascii{reveal} run, $\sigma_i$, is published on $\E$, and $\ascii{Ver}(PK,m_i,\sigma_i) = \emph{true}$. However, if $tout_{rev}^i$ seconds pass before this happens, then the stage fails. In the successful case, if $i<l$, then $\E$ continues to the ($i+1$)th pending stage, otherwise, $i=l$ and $\E$ enters the final stage. In case of failure, $\E$ enters the abort stage.
        
        \item[Final] The final stage indicates that the EVR source has completed successfully.
        
        \item[Abort] The abort stage indicates that the EVR source has failed. In this stage, any future call to any of $\E$'s functions fails.
\end{description}

$\E$ satisfies the following properties: 
\begin{description}
    \item[Non-triviality] The commit stage ends successfully. 
    
    \item[Secrecy] If the commit stage ends successfully, then for all $1 \le i \le l$, during the $i$th pending stage, no user obtains $\sigma_i$. 

    \item[Robustness] If the commit stage ends successfully, then $\E$ reaches the final stage.
\end{description}
\end{definition}


\begin{definition}[Multi-Shot EVR Correct-Usage]
\label{def:multi_evrs-usage}
A correct consumer of a multi-shot EVR source sets a list of $l$ verifiable conditions, $(cnd_1,\dots,cnd_l)$, that all mature at some point, and satisfies the same conditions as in \Cref{def:evrs-usage}.
% \begin{enumerate}[label=MS-CU\arabic*.,ref=MS-CU\arabic*]
    
%     \item If non-triviality breaks, no user gains illicit profit.\label{def:multi_evrs-usage:commit}
    
%     \item If robustness breaks, the total illicit profit gained by all users is at most $P$.\label{def:multi_evrs-usage:reveal}
    
%     \item If secrecy breaks, the total illicit profit gained by all users is at most $P$.\label{def:multi_evrs-usage:before_cnd}
    
%     \item If secrecy and robustness are preserved, no user gains illicit profit.\label{def:multi_evrs-usage:after_cnd}

% \end{enumerate}
\end{definition}

% Remark: 
% Note that we restrict $l < \infty$, even though in some cases (e.g., blockchains) random values are perpetually generated. Fundamentally, no entity can participate for unlimited time nor afford an endless execution of the EVR source until getting paid. Therefore, in these cases randomness generation should be split into segments, where in each segment a fresh EVR source is initiated and $l \in \mathbb{N}$ random values are produced. If the set of EVRS' participants is fixed, then redoing the \ascii{commit} procedure is unnecessary. Surly, further optimizations can be made when executing several multi-shot EVRSs in sequence, but we leave it for future work.


==> trash/prototype_implementation.tex <==
To show our construction is practical, we provide the missing details required to implement a multi-shot EVR source in Ethereum.
% There are some evident differences between Ethereum and our somewhat simplified economic environment.

\paragraph{Ethereum.}
In our model, we formulate a somewhat simplified economic environment. In particular, writing to $\Z$ is free of charge, transactions are appended to the Log immediately after being issued,
% and if a few transactions arrive together they are ordered in a random fashion
and the number of transactions that can be appended to the Log in every \red{step} is unlimited. 
However, in Ethereum, transactions are appended for a fee, miners order transactions \red{at will}, and a transaction block is confined to a maximum number of operations; thereby, a block can only contain a limited number of transactions. Basic operations are measured in gas, a unit of measurement quantifying the computational resources an operation consumes. So, a transaction fee is calculated according to the gas its operations consume multiplied by the gas cost set by its issuer. Currently, an Ethereum block is limited at a maximum of $\sim$10,000,000 gas in total. 
\red{Why is this paragraph necessary?}


\paragraph{The commit stage.} In the commit stage, the Eth-DKG protocol takes place where a DKG protocol is performed among the registered participants (see more details in \Cref{sec:eth_DKG}). At the center of Eth-DKG protocol is an Ethereum smart contract that oversees a correct execution of the protocol and incentivizes the participants to act appropriately. Therefore, it is trivial to incorporate Eth-DKG in our EVR source implementation. As required from the specification of a multi-shot EVR source, Eth-DKG installs a VRF by employing a threshold BLS signature scheme.
To evaluate the VRF, a quorum of investors needs to gather all its members' BLS signatures and reconstruct the threshold signature. BLS signature operations are performed through designated precompiled contracts (see~\cite{ethereum}, App. E) that utilize specific elliptic curve groups for gas efficiency. For further details see~\cite{rational-threshold-cryptposystems}.
\red{I think the paragraph is a bit long. Our point here is that it's not trivial to implement a VRF's \ascii{ver} algorithm on-chain efficiently.}

\paragraph{Framing.} Unfortunately, a straightforward implementation of framing, by publishing a framing transaction with the secret (a group signature), is susceptible to a front-running attack. Namely, prior to its inclusion in the blockchain, an attacker can snatch the secret and inject its own framing transaction beforehand.
Our implementation addresses this issue by dividing \ascii{framing} into a two-phase commit-reveal scheme, as we illustrate in \Cref{fig:framing_ethereum}. In the first phase, the framer sends the contract a hash of the secret concatenated with its $pk$. In the second phase, the framer reveals to the contract the secret along with its $pk$. At that point, the contract verifies that the secret concatenated with $pk$ matches the formerly published hash, and in the case of an authentic secret, the contract pays $pk$. Note that in order to mitigate chain reorganization attacks, the framer has to wait for some blocks to accumulate between the two phases. However, this facilitates delay attacks in which a malicious user can submit a false framing transaction in the first phase, without the intention (or competence) to reveal the real secret on the second phase. Therefore, to disincentivize such attacks, a framer is required to submit an additional deposit in the first phase as a pledge to reveal the authentic secret later on. 
% to disincentive investors from submitting false framing commitments that hamper the protocol's progress, each framer submits an additional deposit when committing.

%  Cite submarine paper....
% \footnote{We note that, chain reorganization attack can also be used to steal a framing reward. There, an attacker reverts an already appended framing transaction and slips its own framing transaction with the observed secret. Therefore, when using a commit-reveal scheme the framer have to wait for some blocks to accumulate between the two phases}

\input{figures/framing_ethereum}

\paragraph{Transaction fees.}
\sout{Since the simple EVR solution disregards transaction fees, in practice, an investor playing the default strategy will end up in a \red{deficit}. This invalidates our game-theoretic analysis and would undermine secrecy and robustness.} \red{I'd open: Our blockchain abstraction and our analysis ignore transaction fees. The issue of transaction fees arises in the reveal transaction -- the investor that submits it pays the fee. This creates a situation where one of the investors must be altruistic about this. In most cases, transaction fees are negligible, and it is quite reasonable to ignore this concern. However, we can do better...} To address this issue, the EVR's consumer fully reimburses investors' transaction fees (possibly by delegating part of the jackpot), but only up to a maximum gas cost. 
% we describe next a rather simple mechanism for subsidizing investors gas fees by the EVR's consumer. The consumer fully recompenses  Possibly by delegating part of the jackpot
% The consumer recompenses investor's transaction fee, but only up to a maximum gas cost. 
Investors' reimbursement is settled in the final stage of the EVR source. Note that Solidity, Ethereum dominant smart contracts language, provides the necessary operations to compute a transaction's gas cost (\ascii{tx.gasprice}$\red{()}$) and the total amount of gas it consumed (\ascii{\red{tx.}gasleft}$()$).
Apart from recouping investors' profits, this simple solution exhibits a few more merits. First, it puts a cap on the consumer's expenses, guaranteeing its coins (or jackpot) are not being siphoned off. Second, it reduces investors' motivation to act strategically in cases where only some of the investors are necessary to send a transaction (for instance, when revealing the secret).
% when there are transactions that only a portion of the investors have to send this procedure guarantees a fair game - prevents "game of chicken". 
Last, it incentivizes investors to set their transaction gas costs according to whatever the consumer determined. Since, by and large, Ethereum transactions are queued in decreasing order of their gas cost, it gives the consumer some level of control on the pace by which the EVR source progresses. 

\paragraph{Congestions.} Nonetheless, the Ethereum network is notorious for its frequent congestion periods, which are characterized by exorbitant gas costs. In such periods, the consumer will not be able to subsidize transaction fees, consequently slowing down randomness publication. Conveniently, GasToken~\cite{GasToken} is a rather sophisticated technique that enables, at least conceptually, to purchase gas, store it, and later on consume it to cover transaction fees. Hence, by buying gas in low gas-cost periods, the EVR source can remain stable, continuously providing random values, even in (not too long) periods of congestion.

% in low gas-cost periods for future use. Hence, GasToken the EVR source can remain stable, continuously providing random values, even in (not too long) periods of congestion.



\paragraph{Timeouts.} To guarantee progress, we conventionally incorporate timeouts into the specification of the EVRS smart contract. As a general rule, timeouts are measured by blocks number. Typically, setting timeouts correctly is a difficult task. A timeout needs to be long enough to give everyone enough time to submit their transactions, especially in the case of a denial of service attack. On the contrary, setting the timeout too long can cause responsiveness issues by allowing an attacker to delay the protocol.
\red{I think that this isn't done?}

    




==> trash/related_work.tex <==
The problem of distributed randomness in economic contexts appears in many protocols and systems. Still, there is not a single agreed-upon way to frame this problem and ponder about it, and there are not conventional criteria to evaluate different solutions against. In this section we compare several approaches to tackle this problem, our solution among them. 

The systems that fall under our lens have 2 properties:
\begin{enumerate}
    \item An economic outcome is governed by a random process. That is, some of the system's participants make a profit, and other lose, according to the outcome of a random process.
    \item The randomness is not provided by a trusted party, but by the system's participants themselves.  
\end{enumerate}
Obviously, since there are many such systems out there, we will relate only to a selected few. 

While systems can vary within this class quite vastly, we are able to define certain criteria over which these systems make trade-offs. \emph{Fairness} is the first criterion we consider, where some systems have absolute fairness and others are fair only under certain assumptions and scenarios, e.g., economic fairness means that fairness can only be guaranteed to the extent that if it was violated the entity that caused the violation lost money. The second criterion is \emph{pragmatism} which takes into account different practical considerations in implementing a system. Finally, we consider \emph{Randomness-as-a-Service} which loosely speaking measures how trustworthy a protocol is to a bystander who is not actively taking part of the randomness generation process.

\subsection{Fairness}
A system is fair to the extent that it can guarantee to an honest participant (i.e., one that adheres to the system's rules) their expected net earnings given a specific set of decisions they make within the system, and regardless of other users' decisions (even if they violate the game's rules). The best example is a simple lottery -- every ticket should entitle its owner to an equal winning probability of the jackpot. Generally speaking, there are 2 ways to break the fairness of a system:
\begin{enumerate}
    \item Distortion. The random process is distorted before it is revealed to the component of the system that is responsible to allocate prizes to winners. Of course, we are interested in meaningful distortion that is done in favor of the distorting party. In the lottery example this can be done in 2 ways: a participant that obtains the result of the random process buys the matching winning ticket; or a user that has a ticket manipulates the random process until they win. 
    \item Robustness. The random process or outcome is indefinitely hidden from the component of the system that is responsible to allocate prizes to winners. Every system then needs to decide how it allocates prizes and when. It might be quite hard to guarantee the allocation of prizes to winners in this scenario (surprisingly it is actually possible). Of course, we are interested in meaningful failures of robustness, where the parties that fail robustness do so when they are aware of their loss.
\end{enumerate}
Some systems guarantee fairness under no assumptions what so ever. For instance, Bentov and Miller's zero-collateral $n$-player tournament-like lottery over Bitcoin or Ethereum (\cite{zero_collateral_lotteries}). Here, the fairness comes on the expense of excessive interaction between users. Bentov et al. also provide absolute fairness in their commit-reveal lottery (\cite{bitcoin_fair_lottery, MPC_bitcoin}), but under a very high collateral that must accompany every purchased ticket.

In Bitcoin things are a bit different. Robustness in Bitcoin is very strongly guaranteed, but distortion of the random process is more of a concern. Large miners can adopt mining strategies that deprive honest miners from their profits and increase their expected profitability above the system's specifications. In Algorand a similar problem exits.

RANDAO, a coin toss protocol over Ethereum with deposits and penalties is a system where distortion is impossible, but robustness is tricky -- it is enough that a single participant refuses to publish a single commitment for the scheme to fail. Of course, the participant that refuses to reveal, referred to as the ``last actor'', does so after she has locally computed the result (and apparently did not like it). This actor is penalized, which is a good start to discourage them from doing so, but still they might be at a profit relative to revealing their share. 

Another way to tackle the last actor problem is to install a threshold cryptosystem on top of the individual commitments \red{(as done for example in ~\cite{})}. In essence, each participant distributes shares to the other participants such that enough of them can open her commitment if they cooperate. Thus, a last actor can be forced to open her commitment if she fails to do so willingly.

Our solution is in its basis a coin tossing protocol, but it cleverly combines the two -- a threshold cryptosystem, and deposits and penalties. Dfinity~\cite{} and \red{Ouroboros?~\cite{}} proposed the closest related protocols but they are not fully specified so we cannot include them in our comparison. Our incentive layer, which sets a restriction on the prizes that can be allocated and introduces framing rewards defines a sweet spot in which robustness and distortion are not stable outcomes, while the minimal collateral put by a participant is $O(1)$ and the prizes that can be allocated are only bounded by the amount of participants.

\subsection{Practical Considerations}
In this section we discuss how practical each system is. Here we relate to a single end-to-end run of the system, and consider the communication complexity, the costs, the time etc. We take into account the infrastructure on top of which the system is built and take its limitations into account. We also compare what each system expects of its users, and what responsibilities they posses.
\red{On-demand vs beacon systems?} 

\subsection{Randomness-as-a-Service}
Fairness is considered when the participants that generate the randomness are also the ones impacted by it. In this section we reflect on the ability of systems to stay trustworthy when the set of participants that generate the randomness and the set of participants that are impacted by it are different. Put differently, fairness talks about private randomness and here we consider public randomness.

One class of protocols that produce trustworthy public randomness rely on delayed computation. Bitcoin, which builds a clever incentive mechanism on top of a Proofs-of-Work system, is a good example. Ethereum's forthcoming VDF-based randomness beacon is another example. These systems are first and foremost leader election protocols, but as a by product, they can be seen as randomness beacons that regularly emit random bits. The smart contract presented in~\cite{proof_of_delay_ethereum} that implements a randomness beacon from a hash-chain is yet another example of how publicly trustworthy random bits can be produced with delayed computation.

All of these systems are based on a similar structure -- the random process amounts to executing a time consuming task whose outcome is unknown at the time when the task is defined. Generally, whoever completed the task can prove it publicly and they are incentivized to so, as fast as possible, for a prize. Once they do, the next task is defined.

In all of these systems there are 2 principal factors that make the random bits publicly trustworthy:
\begin{enumerate}
    \item Open participation and evaluation. Anyone can take part in executing the task, and anyone can verify (cheaply and quickly) that a task was indeed executed correctly when someone claims to have completed it. 
    \item Distortion cost. Anyone that completed a task and refuses to reveal it, pays a cost, that can be evaluated quite accurately. This cost is inherent can cannot be avoided.  
\end{enumerate}

Classical commit-reveal schemes are generally less reliable as a public source of randomness, just because if the set of processes that actually contribute to the randomness process are cooperating they can easily and with zero cost distort the ``random bits'' at they please.

However, in systems like Algorand~\cite{} and Dfinity~\cite{}, and in general in Proof-of-Stake systems which are very open, non-computationally intensive randomness generation processes seem to be trustworthy and the reason is that cooperation on a very large scale between a very large of independent entities is non feasible. In our context we thus need to make sure that our registration phase enables a very large amount of registrations. Of course, the problem is how you make sure that not too many of these registrations are made by the same entity.  

We also check the decentralization potential of a system -- how open the system is for anyone to take part in the randomness generation process, do you have to be a professional to do so, how costly it is to participate (opportunity cost for deposits vs total cost for mining), is there collusion pressure for independent entities to join forces.    




